Towards the decentralized coordination of multiple self-adaptive systems

When multiple self-adaptive systems share the same environment and have common goals, they may coordinate their adaptations at runtime to avoid conflicts and to satisfy their goals. There are two approaches to coordination. (1) Logically centralized, where a supervisor has complete control over the individual self-adaptive systems. Such approach is infeasible when the systems have different owners or administrative domains. (2) Logically decentralized, where coordination is achieved through direct interactions. Because the individual systems have control over the information they share, decentralized coordination accommodates multiple administrative domains. However, existing techniques do not account simultaneously for both local concerns, e.g., preferences, and shared concerns, e.g., conflicts, which may lead to goals not being achieved as expected. Our idea to address this shortcoming is to express both types of concerns within the same constraint optimization problem. We propose CoADAPT, a decentralized coordination technique introducing two types of constraints: preference constraints, expressing local concerns, and consistency constraints, expressing shared concerns. At runtime, the problem is solved in a decentralized way using distributed constraint optimization algorithms implemented by each self-adaptive system. As a first step in realizing CoADAPT, we focus in this work on the coordination of adaptation planning strategies, traditionally addressed only with centralized techniques. We show the feasibility of CoADAPT in an exemplar from cloud computing and analyze experimentally its scalability.

==> figures/conceptualarch_v4.tex <==
%% \newcommand{\drawfullsas}[3]{
%%   \node [managingsys] (Managing#1) at (#2, #3) {Managing subsystem $c_{#1} \in C_{#1}$ $o_{#1} \in O_{#1}$ $k_{#1} \in K_{#1}$};
%%   \node[managedsys, below=of Managing#1] (Managed#1) {Managed subsystem $s_{#1} \in S_{#1}$};
%%   \node[above=1ex of Managing#1] (Label#1) {SAS#1};
%%   \node [draw, inner sep=1ex, fit=(Managing#1) (Managed#1) (Label#1)] (SAS#1) {};

%%   \draw ($ (Managing#1.south) + (-4ex, 0) $)  to ($ (Managed#1.north) + (-4ex, 0) $);
%%   \draw ($ (Managing#1.south) + (4ex, 0) $)  to ($ (Managed#1.north) + (4ex, 0) $);
%% }

%% \newcommand{\filesymbol}[1]{
%%   \begin{tikzpicture}[scale=#1]
%%     \draw (0,0) rectangle (1,1);
%%     \draw (0.2,0.8) -- (0.8,0.8);
%%     \draw (0.2,0.6) -- (0.8,0.6);
%%     \draw (0.2,0.4) -- (0.8,0.4);
%%     \draw (0.2,0.2) -- (0.8,0.2);
%%   \end{tikzpicture}
%%}

\newcommand{\drawfullsasB}[4]{
  %%   \node [managingsys] (Managing#1) at (#2, #3) {Managing subsystem $c_{#1} \in C_{#1}$ $o_{#1} \in O_{#1}$ $k_{#1} \in K_{#1}$};
%%   \node at ($ (#2, #3) + (0, 6ex) $) (Policy#1) {\filesymbol{1.5em}{1.75em}};

  \node[managingsys, minimum height=6ex, align=left, inner ysep=1ex] at (#2, #3) (Logic#1) {};
  \node[managinglabel, align=right, right=-12.5ex of Logic#1] {Adaptation logic};
%%   \node[inner sep=0.25ex] at ($ (#2, #3) + (0.75, 0) $) (Policy#1) {\filesymbol{1.2em}{1.75em}};
  \node[strat] at ($ (#2, #3) + (-0.75, 0.1) $) (Policy#1) {{#4}3};
  \node[below=-0.6ex of Policy#1, font=\scriptsize] {Active strategy};


%%   \node[above=2ex of Logic#1, inner sep=0.25ex] (Policy#1) {\filesymbol{1.5em}{1.75em}};
%%   \node[managingsys, above=2ex of Policy#1] (PolicyMan#1) {Policy management};

  \node[managingsys, minimum height=13ex, align=left, above=of Logic#1] (PolicyMan#1) {};
  \node[managinglabel, text width=3em, right=-8.5ex of PolicyMan#1, align=right] {Planning strategy manager};
  \node[inner sep=0, above=0.5ex of PolicyMan#1] (ManagingLabel#1) {Managing system};

  \node[strat, left=-5ex of PolicyMan#1] (StratM#1) {{#4}2};
  \node[strat, above=1ex of StratM#1] (StratT#1) {{#4}1};
  \node[strat, below=1ex of StratM#1] (StratB#1) {{#4}3};

  \node[draw, minimum width=5em, xshift=1.2em, dashed, inner ysep=1ex, fit=(StratM#1) (StratT#1) (StratB#1)] (StratSelect#1) {};
  \node[font=\scriptsize, anchor=base, right=-3ex of StratSelect#1] {\rotatebox{90}{Strategy selection}};

  \draw (StratB#1.east) -| ($ (StratSelect#1.south) + (1ex, 0)$)  node (StratInt#1) {};
  \draw[-{Latex[fill=black]}] (PolicyMan#1.west) to ($(StratB#1.west) + (0.25ex, 0)$);

%%   \node[managedsys, below=of Managing#1] (Managed#1) {Managed subsystem $s_{#1} \in S_{#1}$};

  \pgfsetlayers{bg,bg2,main}
  \begin{pgfonlayer}{bg2}
    \node[managingsys, inner xsep=1ex, fit=(Logic#1) (PolicyMan#1) (ManagingLabel#1)] (Managing#1) {};
  \end{pgfonlayer}

  \path let
  \p1=(Managing#1.west),
  \p2=(Managing#1.east)
  in node [
    managedsys,
    minimum width=\x2-\x1,
    below=2ex of Managing#1,
  ] (Managed#1) {Managed element};

%%   \node[managedsys, below=of Managing#1] (Managed#1) {Managed subsystem};
  \node[above=0.25ex of Managing#1, text width=6em, align=center] (Label#1) {SAS #4};

  \begin{pgfonlayer}{bg}
    \node[draw, fill=black!5, inner sep=0.75ex, fit=(Managing#1) (Managed#1) (Label#1)] (SAS#1) {};
  \end{pgfonlayer}

%%   \node[right=0ex of Policy#1] {Policy};

  \draw[{Latex[fill=black]}-] ($ (Logic#1.south) + (-8ex, 0) $)  to node[arrowlabel, midway, right] {monitor} ($ (Managed#1.north) + (-8ex, 0) $);
  \draw[-{Latex[fill=black]}] ($ (Logic#1.south) + (8ex, 0) $)  to node[arrowlabel, midway, left] {adapt} ($ (Managed#1.north) + (8ex, 0) $);

%%   \draw[{Latex[fill=black]}-{Latex[fill=black]}] (Logic#1) to (Managed#1);
%%   \draw[{Latex[fill=black]}-{Latex[fill=black]}] (Policy#1) to (Logic#1);
  \draw[{Latex[fill=black]}-] (Policy#1) to node[arrowlabel, pos=0.65, left] {assign} (PolicyMan#1.south -| Policy#1.north);
  \draw[{Latex[fill=black]}-] ($ (PolicyMan#1.south) + (8ex, 0) $) -- node[arrowlabel, midway, left] {monitor} ($ (Logic#1.north) + (8ex, 0) $);
  \draw (StratInt#1.center) to (PolicyMan#1.south -| Policy#1.north);
%%   \draw[{Latex[fill=black]}-{Latex[fill=black]}] (Policy#1) to (PolicyMan#1);
}


\newcommand{\drawfullsas}[4]{
  %%   \node [managingsys] (Managing#1) at (#2, #3) {Managing subsystem $c_{#1} \in C_{#1}$ $o_{#1} \in O_{#1}$ $k_{#1} \in K_{#1}$};
%%   \node at ($ (#2, #3) + (0, 6ex) $) (Policy#1) {\filesymbol{1.5em}{1.75em}};

  \node[managingsys, minimum height=6ex, align=left, inner ysep=1ex] at (#2, #3) (Logic#1) {};
  \node[managinglabel, left=-12.5ex of Logic#1] {Adaptation logic};
%%   \node[inner sep=0.25ex] at ($ (#2, #3) + (0.75, 0) $) (Policy#1) {\filesymbol{1.2em}{1.75em}};
  \node[strat] at ($ (#2, #3) + (0.75, 0.1) $) (Policy#1) {{#4}1};
  \node[below=-0.6ex of Policy#1, font=\scriptsize] {Active strategy};


%%   \node[above=2ex of Logic#1, inner sep=0.25ex] (Policy#1) {\filesymbol{1.5em}{1.75em}};
%%   \node[managingsys, above=2ex of Policy#1] (PolicyMan#1) {Policy management};

  \node[managingsys, minimum height=13ex, align=left, above=of Logic#1] (PolicyMan#1) {};
  \node[managinglabel, text width=3em, left=-8.5ex of PolicyMan#1] {Planning strategy manager};
  \node[inner sep=0, above=0.5ex of PolicyMan#1] (ManagingLabel#1) {Managing system};

  \node[strat, right=-5ex of PolicyMan#1] (StratM#1) {{#4}2};
  \node[strat, above=1ex of StratM#1] (StratT#1) {{#4}1};
  \node[strat, below=1ex of StratM#1] (StratB#1) {{#4}3};

  \node[draw, minimum width=5em, xshift=-1.2em, dashed, inner ysep=1ex, fit=(StratM#1) (StratT#1) (StratB#1)] (StratSelect#1) {};
  \node[font=\scriptsize, anchor=base, left=-3ex of StratSelect#1] {\rotatebox{90}{Strategy selection}};

  \draw (StratT#1.west) -| ($ (StratSelect#1.south) + (-1ex, 0)$)  node (StratInt#1) {};
  \draw[-{Latex[fill=black]}] (PolicyMan#1.east) to ($(StratT#1.east) + (-0.25ex, 0)$);

%%   \node[managedsys, below=of Managing#1] (Managed#1) {Managed subsystem $s_{#1} \in S_{#1}$};

  \pgfsetlayers{bg,bg2,main}
  \begin{pgfonlayer}{bg2}
    \node[managingsys, inner xsep=1ex, fit=(Logic#1) (PolicyMan#1) (ManagingLabel#1)] (Managing#1) {};
  \end{pgfonlayer}

  \path let
  \p1=(Managing#1.west),
  \p2=(Managing#1.east)
  in node [
    managedsys,
    minimum width=\x2-\x1,
    below=2ex of Managing#1,
  ] (Managed#1) {Managed element};

%%   \node[managedsys, below=of Managing#1] (Managed#1) {Managed subsystem};
  \node[above=0.25ex of Managing#1, text width=6em, align=center] (Label#1) {SAS #4};

  \begin{pgfonlayer}{bg}
    \node[draw, fill=black!5, inner sep=0.75ex, fit=(Managing#1) (Managed#1) (Label#1)] (SAS#1) {};
  \end{pgfonlayer}

%%   \node[right=0ex of Policy#1] {Policy};

  \draw[{Latex[fill=black]}-] ($ (Logic#1.south) + (-8ex, 0) $)  to node[arrowlabel, midway, right] {monitor} ($ (Managed#1.north) + (-8ex, 0) $);
  \draw[-{Latex[fill=black]}] ($ (Logic#1.south) + (8ex, 0) $)  to node[arrowlabel, midway, left] {adapt} ($ (Managed#1.north) + (8ex, 0) $);

%%   \draw[{Latex[fill=black]}-{Latex[fill=black]}] (Logic#1) to (Managed#1);
%%   \draw[{Latex[fill=black]}-{Latex[fill=black]}] (Policy#1) to (Logic#1);
  \draw[{Latex[fill=black]}-] (Policy#1) to node[arrowlabel, pos=0.65, right] {assign} (PolicyMan#1.south -| Policy#1.north);
  \draw[{Latex[fill=black]}-] ($ (PolicyMan#1.south) + (-8ex, 0) $) -- node[arrowlabel, midway, right] {monitor} ($ (Logic#1.north) + (-8ex, 0) $);
  \draw (StratInt#1.center) to (PolicyMan#1.south -| Policy#1.north);
%%   \draw[{Latex[fill=black]}-{Latex[fill=black]}] (Policy#1) to (PolicyMan#1);
}

\newcommand{\drawline}[1]{
  \draw[layersep] ($ (SAS2.south east) + (0.05, #1) $) -- ($ (SAS1.south west) + (-2, #1) $);
}

\begin{tikzpicture}[
  scale=1.0,
  transform shape,
  shift=(current page.center),
  node distance=4ex and 2ex,
  font=\rmfamily\footnotesize,
  managedsys/.style={
    draw,
    text width=8em,
    align=center,
    node distance=3ex and 2ex,
    fill=white
  },
  managingsys/.style={
    draw,
    align=center,
    text width=5em,
    node distance=3ex and 2ex,
    minimum width=8.75em,
    fill=white,
    inner xsep=0.5ex
  },
  layersep/.style={
    dashed,
    draw=black!50
  },
  strat/.style={
    draw,
    font=\scriptsize,
    text width=0.8em,
    align=center
  },
  levellabel/.style={
    text width=5em,
    align=left,
    font=\footnotesize
  },
  managinglabel/.style={
    text width=5em,
    align=left
  },
  arrowlabel/.style={
    font=\scriptsize
  },
  smallsas/.style={
    fill=black!5,
    draw
  },
  ]
%%   labelstyle/.style={
%%     text width=6em,
%%   },
%%   boxstyle/.style={
%%     align=center,
%%     text width=4.5em,
%%     % minimum height=8ex,
%%     % node distance=5ex and 4ex,
%%     node distance=15ex and 20ex,
%%     inner ysep=2ex,
%%     inner xsep=0ex,
%%     draw
%%   },
%%   coadaptstyle/.style={
%%     align=center,
%%     text width=6em,
%%     minimum height=3ex,
%%     node distance=4ex,
%%     outer sep=0ex,
%%     draw,
%%     fill=black!15
%%   },
%%   inputstyle/.style={
%% %%     trapezium,
%% %%     trapezium left angle=80,
%% %%     trapezium right angle=100,
%%     align=center,
%%     text width=8em,
%%     minimum height=3ex,
%%     minimum width=5em,
%%     node distance=4ex,
%%     outer xsep=1ex,
%%     draw=black!50,
%%     font=\scriptsize
%%   },
%%   coadaptstylesmall/.style={
%%     coadaptstyle,
%%     font=\scriptsize,
%%     minimum height=2ex,
%%     text width=4.5em,
%%   },
%%   relationstyle/.style={
%%     -Latex[fill=black]
%%   },
%%   relationstylepc/.style={
%%     -Latex[fill=black],
%%     dashed
%%   },
%%   mapestyle/.style={
%%     rectangle,
%%     font=\footnotesize,
%%     text width=2em,
%%     minimum height=4ex,
%%     minimum width=4ex,
%%     draw,
%%     fill=white,
%%     align=center
%%   },

%% ]

%%   \node[managingsys] (Managing1) at (0, 0) {Managing subsystem $c_1 \in C_1$ $o_1 \in O_1$ $k_1 \in K_1$};
  %%   \node[managedsys, below=of Managing1] (Managed1) {Managed subsystem $s_1 \in S_1$};

  \drawfullsas{1}{0}{0}{A}
  \drawfullsasB{2}{5}{0}{B}


%%     \path let
%%     \p1=(SAS1.west),
%%     \p2=(SAS2.east)
%%     in node [
%%       draw,
%%       minimum width=\x2-\x1,
%%       minimum height=8ex,
%%       anchor=west
  %%     ] (Goals) at (\x1, 3) {};

%%   \path let
%%   \p1=(SAS1.west),
%%   \p2=(SAS2.east)
%%   in node [
%%     draw,
%%     minimum width=\x2-\x1,
%%     minimum height=5ex,
%%     anchor=west
%%   ] (Environment) at (\x1, -2.75) {Environment} ;



%%   \draw[{Latex[fill=black]}-{Latex[fill=black]}] (SAS1.south) -- (Environment.north -| SAS1.south);
%%   \draw[{Latex[fill=black]}-{Latex[fill=black]}] (SAS2.south) -- (Environment.north -| SAS2.south);
%%   \draw[{Latex[fill=black]}-{Latex[fill=black]}] (Logic1) -- node[midway,above] {coordinate} (Logic2);
  \draw (PolicyMan1) -- node[text width=4em, align=center, midway,above] {coordinate strategy selection} node[midway, below, text width=4em, align=center] {with \scriptsize\textbf{\CoordDCOP}} (PolicyMan2);

%%   \draw[{Latex[fill=black]}-] ($ (SAS1.south) + (-8ex, 0) $)  to node[arrowlabel, right] {monitor} (\tikztostart |- Environment.north);
%%   \draw[-{Latex[fill=black]}] ($ (SAS1.south) + (8ex, 0) $)  to node[arrowlabel, left] {affect} (\tikztostart |- Environment.north);
%%   \draw[{Latex[fill=black]}-] ($ (SAS2.south) + (-8ex, 0) $)  to node[arrowlabel, right] {monitor} (\tikztostart |- Environment.north);
%%   \draw[-{Latex[fill=black]}] ($ (SAS2.south) + (8ex, 0) $)  to node[arrowlabel, left] {affect} (\tikztostart |- Environment.north);

%%   \drawline{-0.3}
%%   \drawline{1.10}
%%   \drawline{2.7}

%%   \node[levellabel, left=0ex of Environment] (EnvLevel) {Environment level};
%%   \node[levellabel, above=0.7 of EnvLevel] (ManagedLevel) {Managed elem. level};
%%   \node[levellabel, above=0.7 of ManagedLevel] (LogicLevel) {Adaptation logic level};
%%   \node[levellabel, above=0.7 of LogicLevel] (PolicyLevel) {Strategy management level};

  %%   \node[levellabel, text width=12em, draw, dashed, below=0.25 of Environment,fill=black!5, font=\scriptsize] {\textbf{Legend:\ \ \ }\raisebox{-4pt}{\filesymbol{1.0em}{1.55em}} = Strategy specification};

  \node[smallsas] (SASA) at (0, -2.25) {SAS A};
  \node[smallsas] (SASB) at (5, -2.25) {SAS B};
  \node[smallsas] (SASC) at (5, -3.25) {SAS C};
  \node[smallsas] (SASD) at (-1, -3.25) {SAS D};
  \node[smallsas] (SASE) at (1, -3.25) {SAS E};

  \draw[{Latex[fill=black]}-{Latex[fill=black]}] (SASA) to (SASB);
  \draw[{Latex[fill=black]}-{Latex[fill=black]}] (SASB) to (SASC);
  \draw[{Latex[fill=black]}-{Latex[fill=black]}] (SASD) to (SASE);
  \draw[{Latex[fill=black]}-{Latex[fill=black]}] (SASD) to (SASA);
  \draw[{Latex[fill=black]}-{Latex[fill=black]}] (SASE) to (SASA);

%%   \draw[{Latex[fill=black]}-{Latex[fill=black]}] (SASA) to node[font=\scriptsize,midway, above] {\textbf{\CoordDCOP}} (SASB);
%%   \draw[{Latex[fill=black]}-{Latex[fill=black]}] (SASB) to node[font=\scriptsize,midway, right] {\textbf{\CoordDCOP}} (SASC);
%%   \draw[{Latex[fill=black]}-{Latex[fill=black]}] (SASD) to node[font=\scriptsize,midway, above] {\textbf{\CoordDCOP}} (SASE);
%%   \draw[{Latex[fill=black]}-{Latex[fill=black]}] (SASD) to node[font=\scriptsize,midway, left] {\textbf{\CoordDCOP}} (SASA);
%%   \draw[{Latex[fill=black]}-{Latex[fill=black]}] (SASE) to node[font=\scriptsize,midway, right] {\textbf{\CoordDCOP}} (SASA);

  %%   \draw[{Latex[fill=black]}-{Latex[fill=black]}] (SASE) to (SASC);

  \draw[dashed] (SAS1.south west) to (SASA.north west);
  \draw[dashed] (SAS1.south east) to (SASA.north east);

  \draw[dashed] (SAS2.south west) to (SASB.north west);
  \draw[dashed] (SAS2.south east) to (SASB.north east);

\end{tikzpicture}


==> sections/approach.tex <==


\begin{figure*}[t]
  \centering
  % \includegraphics[draft, width=\linewidth, height=6cm]{Figure.pdf}
  \input{figures/conceptualarch_v3.tex}
  \caption{Relation between the \CoordDCOP activities, \ie \ACDCOP for
    analysis coordination and \PCDCOP for \plancoord, and the \mape
    loop. Arrows represent unidirectional flow of information, while
    arrow-less lines and black circles represent multi-directional
    information flow. We used dashed lines to more clearly
    differentiate between \ACDCOP and \PCDCOP.}
  \label{fig:Conceptual}
\end{figure*}

% \begin{figure}[t]
%   \centering
%   % \includegraphics[draft, width=\linewidth, height=6cm]{Figure.pdf}
%   \input{figures/communication_diagram.tex}
%   \caption{Conceptual architecture and interaction sequence of the
%     proposed coordination technique.\am{change ! to $\neg$}}
%   \label{fig:Communication}
% \end{figure}

% \begin{figure*}[t]
%   \centering
%   % \includegraphics[draft, width=\linewidth, height=6cm]{Figure.pdf}
%   \begin{subfigure}{0.4\linewidth}
%   \input{figures/conceptularch_regional.tex}
%   \caption{Conceptual architecture and interaction sequence of the
%     proposed coordination technique.\am{change ! to $\neg$}}
%   \label{fig:Communication}
%   \end{subfigure}
% % \end{figure}

% % \begin{figure}[t]
%   % \centering
%   % \includegraphics[draft, width=\linewidth, height=6cm]{Figure.pdf}
%   \begin{subfigure}{0.4\linewidth}
%   \input{figures/conceptularch_coordinated.tex}
%   \caption{Conceptual architecture and interaction sequence of the
%     proposed coordination technique.\am{change ! to $\neg$}}
%   \label{fig:Communication}
%   \end{subfigure}
% \end{figure*}

% \begin{figure*}[t]
%   \centering
%   \begin{subfigure}[b]{0.5\linewidth}
%   \input{figures/conceptularch_coordinated.tex}
%   \caption{Conceptual architecture...}
%   % \label{fig:Communication}
%   \end{subfigure}%
%   \begin{subfigure}[b]{0.5\linewidth}
%   \input{figures/conceptularch_regional.tex}
%   \caption{Conceptual architecture...}
%   \label{fig:Communication}
%   \end{subfigure}
% \end{figure*}

%% \begin{figure}[t]
%%   \centering
%%   \begin{subfigure}{1.0\linewidth}
%%   \input{figures/conceptularch_coordinated.tex}
%%   \caption{Coordinated control pattern.}
%%   % \label{fig:Communication}
%% \end{subfigure}

%% \vspace{2ex}

%%   \begin{subfigure}{1.0\linewidth}
%%   \input{figures/conceptularch_regional.tex}
%%   \caption{Regional planner pattern.}
%%   % \label{fig:Communication}
%% \end{subfigure}

%% \caption{\todo Replace the figures with something simpler. Coordination with Coord-DCOP (AC-DCOP and PC-DCOP) in two
%%   decentralized \gls{sas} architectures. In the regional planner
%%   pattern, Coord-DCOP realizes coordination in the planning activity,
%%   while in the coordinated control pattern Coord-DCOP supports
%%   coordination in both analysis and planning activities. The
%%   graphical notation is taken from~\cite{Weyns_2013, Quin_2021}.}
%% \end{figure}



\section{Conceptual architecture of \CoordDCOP} \label{sec:ConceptualArch}

In this section we conceptually introduce our coordination technique
for decentralized \gls{sas}, named \CoordDCOP. \CoordDCOP supports
coordination between an arbitrary number of \gls{sas}, and considers
both the analysis \mapef{A} and the planning \mapef{P} activities of
the \mape loop.\am{why only AP?}

We present a conceptual architecture of the technique, followed by how
we concretely realize it for A and P by means of \dcop, which is
presented in Sections X and Y.  \am{somwhere you need to explain: (1)
  DCOP only used for coordination, or do you also use COP for A and
  P?; (2) if so, then you need to justify why realizing A and P via
  COP is a feasible approach (and what may be alternatives and their
  pros/cons}

\subsection{Overview and Steps of \CoordDCOP} \label{sec:ConceptualOverview}

\reffig{fig:Conceptual} depicts the relation between the \mape loop
and \CoordDCOP. \CoordDCOP realizes the coordination of planning
between two or more \glspl{sas} by means of a \glsxtrfull{plancoord}
activity, conceptually extending the \mape loop. During \PCDCOP,
coordinating \glspl{sas} jointly decide on \textit{how} planning
should be carried out, \ie what types of adaptations are allowed, what
are the planning goals, what are the target system states \etc

As depicted in \reffig{fig:Conceptual}, \PCDCOP is decoupled from the
\mapef{P} and exchange of information between \PCDCOP and \mapef{P} is
carried out by means of an \textit{interface}. Decoupling the two
activities means that \PCDCOP can provide \gls{plancoord} regardless
of how \mapef{P} is realized by a particular \gls{sas}
implementation. Moreover, it follows that \PCDCOP allows for each
\gls{sas} participating in \gls{plancoord} to realize their \mapef{P}
activities by means of different techniques, \eg a \gls{sas} realizes
\mapef{P} as \gls{mdp} [cite] and another \gls{sas} realizes \mapef{P}
as search-based planning \cite{Bowers_2018,Shin_2020,Mann_2021}.

The interface to \PCDCOP involves a \textit{forward path} and a
\textit{return path}. The purpose of the \textit{forward path} is to
update \CoordDCOP with the latest system state, coordination objective
(including preferences and requirements), coordination variables,
information about synergies or conflicts \etc In essence, the
\textit{forward path} feeds the necessary input data to
\CoordDCOP. The \textit{return path} simply returns the results of
coordination, \eg how well the coordination objective has been met and
what particular variable setting has been obtained. The results of
\PCDCOP can then be employed in the or \mapef{P}.

\subsection{Elements of \CoordDCOP} \label{sec:ConceptualElements}

\PCDCOP share a number of common concepts. We detail the common
concepts below then specialize them for \PCDCOP in
\refsec{sec:ConceptualPCDCOP}.

\subsubsection{Input to \CoordDCOP}

Because \gls{sas} operate under continuously changing operating
conditions, the coordination setting must also be dynamic. Therefore,
before engaging in a coordination round, the participating \glspl{sas}
must first setup \PCDCOP (the \textit{update} arrow
in \reffig{fig:Conceptual}). Each \mape loop forwards the following
input information to its corresponding \CoordDCOP activities:

\begin{itemize}
\item a list of \textit{\glspl{coordpoint}} and the possible values
  they can take, describing the extent of the joint decision space,
  \eg whether to adapt or not, desired goal state, or allowed
  adaptation actions, among others,
\item a \textit{\gls{coordobjective}} guiding the coordination process
  by ordering the possible assignments of values to \glspl{coordpoint}
  from \textit{best} to \textit{worst}, \eg adapting the managed
  system is preferred to not adapting it,
\item a list of \textit{\glspl{coordpeer}}, \ie references to the
  other \mape loops participating in the coordination, and
\item the \textit{\gls{coordalg}} which must be understood and
  implemented by all \glspl{coordpeer} and which describes how the
  coordination process will take place, \eg what kind of messages will
  be exchanged between \glspl{coordpeer} and in what order.
\end{itemize}

Next some remarks on the above. Firstly, note that the purpose of
coordination is to improve the state of the \gls{sas} from the
perspective of its stakeholders. Therefore, the \gls{coordobjective}
must properly account for stakeholder requirements and
preferences. Moreover, the \gls{coordobjective} must be properly
conditioned on the state of the \gls{sas} and that of its environment
prior to coordination, while also taking into account known sources of
conflicts or synergies between \glspl{coordpoint}, \eg \TODO{example}.

\TODO{Can cite \cite{Lesch_Hadry_2022} who discuss that the selection
  of adaptation planning strategies should depend on the current state
  of the system for best effectiveness.}

%% The \gls{coordobjective} also plays a pbut also on
%% the \textit{expected} state of the system and its environment after
%% coordination. All of these ensure that the results of coordination

Secondly, note that some of the inputs mentioned above can be fixed at
\designtime, while others can indeed vary at \runtime. For example,
fixing the \gls{coordalg} at \designtime is something to be expected
because of implementation overheads, while the \gls{coordobjective} is
closely tied to the system's state therefore it must be updated before
each coordination round, \eg certain decisions make sense only in
certain states or the requirements and preferences of stakeholders
have evolved over time.

Finally, note that the input to \CoordDCOP is characterized by both
local and global aspects. For example, the \gls{coordalg} must be
globally known to all \glspl{coordpeer}. The \gls{coordobjective} is a
global objective, however it can often be decomposed into local
\glspl{subcoordobjective}, \eg the state of the whole system is given
by the state of \texttt{\gls{sas}1} together with that of
\texttt{\gls{sas}2}, where a given sub-objective is the responsibility
to the \glspl{coordpeer} involved in it; such decomposition, if
possible, can reduce the overheads of coordination because a \gls{sas}
does not have to directly coordinate with all of other \glspl{sas},
but only with its direct \textit{neighbors}, \ie \glspl{sas} involved
in the same \gls{subcoordobjective} \cite{Fioretto_2018}. \TODO{revise
  what follows} Implicitly, from the perspective of a \gls{sas}
\texttt{\gls{sas}i}, this has the effect of pruning the lists of
\glspl{coordpeer} down to the \textit{\glspl{directcoordpeer}}, \ie
\glspl{sas} involved in the same \glspl{subcoordobjective} as
\texttt{\gls{sas}i}. Similarly, \glspl{sas} must be aware only of the
those \glspl{coordpoint} under their own control or of the
\glspl{coordpoint} under the control of their \glspl{directcoordpeer}.

\subsubsection{Coordination with \CoordDCOP}

For carrying out the actual coordination, \CoordDCOP, \ie \ACDCOP and
\PCDCOP, employs \dcop algorithms as \gls{coordalg}, which we detail
in Sections \ref{sec:Coord_A} and \ref{sec:Coord_P}.

\subsubsection{Output of \CoordDCOP}

The output of \CoordDCOP is simply the assignment of concrete values
to \glspl{coordpoint}. The output is returned to the other activities
of the corresponding \mape loop.

\TODO{Talk about the similarities between decomposing the
  \gls{coordobjective} and decomposing goals into subgoals. Cite
  \cite{diaconescu2017architectures}}

%% ensures the consistency between \glspl{coordpoint}, \eg a
%% \gls{coordpointAPC} can take the value of \textit{coordinated
%%   adaptation} only if all the others \glspl{coordpointAPC} take the
%% same value or a \gls{coordpointAPC} takes the value \textit{local
%%   adaptation} only if there is at least one \glspl{coordpointA} taking
%% the value \textit{local deviation}. The \gls{coordobjective} must also
%% reflect the current state of the \gls{sas}, \eg if there truly is a
%% deviation from operating goals, then the \textit{no deviation}
%% assignment of a \gls{coordpointAPC} should be \textit{worse} than
%% \textit{global deviation} or \textit{local deviation}. Finally, the
%% \gls{coordobjective} encodes the preferences of stakeholders regarding
%% adaptation, for example stakeholders might strongly prefer
%% \textit{local adaptation} to \textit{coordinated adaptation} in order
%% to avoid further coordination overheads.

\subsection{\Gls{plancoord} with \PCDCOP} \label{sec:ConceptualPCDCOP}

\PCDCOP realizes \textit{\plancoord}. \Gls{plancoord} is an
optimization problem in which \glspl{sas} coordinate on planning
goals, \ie the desired system state, the allowed set of actions, and
the preconditions of those actions before producing individual
adaptation plans \cite{Nissim_2010,Torreno_2017}. An alternative to
\plancoord, is \textit{cooperative planning} where \glspl{sas} jointly
solve a planning problem. We selected \plancoord for \PCDCOP because
it has the advantage of being agnostic to the planners employed by
individual \glspl{sas}; this flexibility is especially important for
multi-stakeholder coordinating \glspl{sas} where individual
\glspl{sas} might be developed by different teams. Moreover,
\plancoord can constitute an input to further cooperative planning
steps. Next we specialize the \glspl{coordpoint} and
\gls{coordobjective} to \PCDCOP.

\subsubsection{\Glspl{coordpoint}}

The \glspl{coordpoint} of \PCDCOP support \plancoord and are of two
types: \textit{\glspl{coordpointPstate}} and
\textit{\glspl{coordpointPaction}}. The \glspl{coordpointPstate}
describe the desired state of the system or of its subsystems, \ie
after coordination, planning, and execution. The
\glspl{coordpointPaction} list the set actions that individual
\glspl{sas} are allowed to employ in adaptation planning, including
their preconditions. Note that the possible concrete values of
\glspl{coordpointPstate} are \glspl{coordpointPaction}
application-specific.

\subsubsection{\Gls{coordobjective}}

As in \ACDCOP, the \gls{coordobjective} of \PCDCOP must ensure the
consistency between \glspl{coordpoint}, while properly representing
the requirements and preferences of \glspl{sas} towards the desired
system state and desired allowed set of actions. To this end, \PCDCOP
considers three types of consistency \glspl{subcoordobjective}:
\textit{\gls{coordconstP}} between \glspl{coordpointPstate} to ensure
the consistency of desired states between \glspl{sas},
\textit{\gls{coordconstPPA}} to ensure the consistency between states
and allowed actions, \textit{\gls{coordconstPA}} to ensure the
consistency of allowed actions pertaining to different \glspl{sas}. In
addition, \PCDCOP also includes two types of preference
\glspl{subcoordobjective}: \textit{\gls{coordconstPpref}} to represent
the preference of \glspl{sas} for certain states and
\textit{\gls{coordconstPApref}} to represent the preference of
\glspl{sas} towards certain action sets.

%% quantifies how \textit{good} a
%% potential system state is, based on the \glspl{coordpointPstate},
%% given stakeholder requirements and preferences. A state violating
%% requirements should never be selected following coordination, while a
%% state meeting stakeholder preferences in the best way possible should
%% always be selected. In addition, the \gls{coordobjective} ensures the
%% consistency between \glspl{coordpointPstate}, \eg to avoid conflicting
%% states between subsystem, the consistency between
%% \glspl{coordpointPaction}, \eg such as to avoid conflicts between
%% adaptation actions, and the consistency between
%% \glspl{coordpointPstate} and \glspl{coordpointPaction}, \eg such as to
%% prune those actions that are incompatible with certain desired states. To match the \PCDCOP for the \gls{coordobjective},

%% \gls{coordconstP} \gls{coordconstPpref} \gls{coordconstPA} \gls{coordconstPApref}


\am{this § is misleading for me; you mentioned that you coordinate among two and more; also why you explain what is not shown?} The two coordination activities mandate the participation of at least
two \gls{sas} and are specified as \glsxtrfullpl{dcop} following the
procedures described in \refsec{sec:Coord_A} and
\refsec{sec:Coord_P}. Note that, while not depicted in
\reffig{fig:Communication}, we allow other means of decentralization,
between an arbitrary number of \gls{sas}, at the level of the
\mapef{M} and \mapef{E} activities. 

\subsection{Application to Running Example}
\am{could be nice to conceptually explain it for the running example}

\section{Realization of \CoordDCOP via \dcop}

In this section we describe the realization of \ACDCOP and \PCDCOP
with \dcop. We start with a brief background on \dcop.

\subsection{Background on \dcop} \label{sec:Back_DCOP}

\Glsxtrfullpl{dcop} \cite{Modi_2005, Nguyen_Yeoh_2019,Fioretto_2018}
involve agents coordinating the value assignments of owned variables
in order to optimize a certain objective function. The multi-agent
system community has studied many applications of \dcops to real-life
problems, such as coordinating \glsxtrshort{iot} devices to minimize
energy consumption in smart grids \cite{fioretto2017multiagent},
coordinating logistic operations using privacy-sensitive means
\cite{leaute2011coordinating}, minimizing congestion in disaster
evacuation scenarios \cite{kinoshita2013effective}, composing web
services in a \gls{qos}-aware manner \cite{Temglit_2018}, placing
application components on \cloud resources \cite{Jin_2011}, or
implementing the self-repair function in networks of physical agents
\cite{rust2020resilient} (\todo maybe remove examples; they also
appear in the introduction).

\dcops are related to the \csp, a kind of formal specification often
employed in the self-adaptive literature \cite{metzger2016coordinated,
  Paz_2016, Oliveira_2013, AlShara_2018, Bruneliere_2018, Song_2013,
  Anders_2015, Vansyckel_2013}. \dcops generalize \csps, \ie by
allowing constraints to take real values instead of, and also extend
them to the distributed or multi-agent setting.

In the multi-agent systems literature
\cite{Nguyen_Yeoh_2019,Fioretto_2018}, a \dcop is defined as a tuple
$\langle \mathbf{X, D, F, A, \pi, \mu} \rangle$, where:

\begin{itemize}
  \item $\mathbf{A} = \{a_1, \dots, a_m\}$ is a set of agents.
  \item $\mathbf{X} = \{x_1, \dots, x_n\}$ is a set of variables.
  \item $\mathbf{D} = \{D_1, \dots, D_n\}$ is a set of finite variable
    domains, with each variable $x_i$ taking values from  $D_i$.
  \item the tuples $(x_i, d_i)$, where $d_i \in D_i$, are
    \textit{value assignments}; the set $\sigma = \{(x_i, d_i) |
    i=1..n\}$ is a \textit{complete assignment} of values to
    variables, while $\sigma_S \subseteq \sigma$ is called a
    \textit{partial assignment}.
  \item $\mathbf{F} = \{c_1, \dots, c_k\}$ is a set of
    \textit{constraint functions}, also known as \textit{cost
      functions} or simply \textit{constraints}, with each $c_i$
    having a scope $S_i \subseteq \mathbf{X}$; the role of a
    constraint is to map a partial assignment $\sigma_{S_i}$ of
    variables from its scope to a real-valued \textit{cost}. An
    important characteristic of a constraint function $c_i$ is its
    \textit{arity}\footnotemark{}, \ie how many variables are part of
    its scope $S_i$.

    \footnotetext{\dcop algorithms usually assume an arity of at most
      two, that is they only operate on \textit{unary} or
      \textit{binary} constraints. There have been extensions proposed
      to algorithms in order to handle n-ary constraints
      \cite{Pecora_2007}.}

      % Another common solution is to pre-process
      % the n-ary constraint into multiple binary or unary ones (cite).}
  \item $\mathbf{\pi} : \mathbf{X} \to \mathbf{A}$ is a function
    mapping variables to agents. If $\pi(x_i) = a_i$, then it means
    that $a_i$ controls how the values from $D_i$ are assigned to
    $x_i$, \ie $a_i$ \textit{controls} or \textit{owns} $x_i$. Note
    that, for algorithmic simplicity, \dcop algorithms usually assume
    that an agent controls a single variable and that a variable is
    controlled by a single agent\footnotemark{}. We follow the same
    assumption in this paper.

    \footnotetext{Techniques to work around this limitation are
      discussed in \cite{Modi_2005,yokoo2012distributed}.}

\item $\mu(\sigma)$ is the \textit{objective function}, where $\sigma$
  is a complete assignment. Usually, the objective function is just
  the sum of costs, \ie $\mathbf{\mu} (\sigma) = \sum_{i=1\dots k}
  c_i(\sigma_{S_i})$.
\end{itemize}

Solving the \dcop means finding an assignment $\sigma^{\star}$ of all
variables from $\mathbf{X}$, which minimizes\footnotemark{} the
objective function $\mu(\sigma)$. Solving a \dcop is known to be
NP-hard \cite{Fioretto_2018, Modi_2005}.

\footnotetext{Note that, for simplicity, all the \dcops discussed in
  this paper aim at minimizing an objective function. However, in
  general, \dcops can also be constructed as maximization problems. In
  maximization \dcops, constraint functions are known as
  \textit{reward functions} or \textit{utility functions}.}

Note that a \dcop is solved in a distributed fashion: agents exchange
messages with their neighbors\footnotemark{}, following certain rules
or \textit{algorithms}, such as to discover the optimal assignment
$\sigma^{\star}$. Starting out as extensions of established discrete
optimization algorithms, \eg SyncBB \cite{hirayama1997distributed}
which extends the branch-and-bound algorithm, many algorithms have
been proposed in the past two decades to solve \dcops, \eg
\cite{petcu2005dpop, Modi_2005, Farinelli_2008}. For a comprehensive
survey on \dcop algorithms, please see \cite{Fioretto_2018}.

\footnotetext{Two agents $a_1$ and $a_2$ controlling variables $x_1$
  and $x_2$ are \textit{neighbors} if $\exists c \in \mathbf{F}$ with
  scope $S$ having the property that $x_1, x_2 \in S$.}

Within decentralized \gls{sas}, \dcop can provide both the formal
language to describe complex coordination problems between multiple
\glspl{sas} and the necessary mechanisms to carry out the coordination
itself. In the case of \CoordDCOP, we can use \dcop variables to
formally specify \glspl{coordpoint}, \dcop constraints to specify the
\gls{coordobjective}, and \dcop agents, implementing certain \dcop
algorithm, to execute the coordination. We elaborate this idea in the
next two sections for \ACDCOP and \PCDCOP.

\subsection{Realizing \ACDCOP with \dcop} \label{sec:Coord_A}

\iffalse
\begin{figure}[t]
  \centering
  % \includegraphics[draft, width=\linewidth, height=6cm]{Figure.pdf}
  \input{figures/analysistypes.tex}
  \caption{Analysis coordination metamodel. \todo Add an ``Agent'' box.}
  \label{fig:AnalysisTypes}
\end{figure}
\fi

We specify \ACDCOP, as introduced in \refsec{sec:ConceptualArch}, using
\dcop as follows. First, we specify \textbf{\glspl{coordpointA}} as
\dcop variables from the set $X_a =\{x_{a1},\dots,x_{an}\} \subseteq
\mathbf{X}$. The domain of each $x_{ai}$ is $D_{ai} =
\{\mathit{cadapt, ladapt, nadapt}\}$, where $\mathit{cadapt}$
corresponds to \textit{coordinated adaptation}, $\mathit{ladapt}$ to
\textit{local adaptation}, and $\mathit{nadapt}$ to \textit{no
  adaptation}.

Next, we specify the \textbf{\gls{coordobjective}} of \ACDCOP using a
\dcop objective function $\mu_{A}$ given by:

\begin{equation}
  \begin{alignedat}{2}
    \mu_{A}(\sigma) = &\quad\mu_{a}(\sigma) &+& \quad\mu_{p}(\sigma) \\
                    = & \sum_{\substack{c_{ai} \in F_a \\ i=1..|F_a|}} c_{ai} (\sigma_{S_{ai}})\, & +&  \sum_{\substack{c_{pi} \in F_p \\ i=1..|F_p|}} c_{pi} (\sigma_{S_{pi}}) \,,
  \end{alignedat}
\end{equation}

where $\mu_{a}(\cdot)$ is the \gls{coordconstA} and $\mu_{p}(\cdot)$
is the \gls{coordconstApref}. $F_a,F_p \subseteq \mathbf{F}$ are sets
of constraints, with $c_{ai} \in F_a$ ensuring the consistency between
two or more \glspl{coordpointA} and $c_{pi} \in F_p$ enforcing
adaptation preferences. $\sigma_{S_{ai}}$ are the assignments of
variables from $X_{ai}$ corresponding to the scopes of the $c_{ai}$
constraints and $\sigma_{S_{pi}}$ are assignments of variables from
$X_{ai}$ corresponding to the scope of the $c_{pi}$. Finally, we
assign to each variable $x_{ai} \in \mathbf{X}$ an agent $a_{ai} \in
\mathbf{A}$. Conceptually, each \gls{sas} involved in \ACDCOP controls
one agent $a_{ai}$ and the \textbf{peers} of \gls{sas} will be
neighboring agents. The \ACDCOP \textbf{algorithm} will be the one
implemented by the agents (see \refsec{sec:ProtoImpl}).

Two remarks: note that $c_{pi}$ are \textit{unary} constraints,
\ie $|S_{pi}| = 1$, and that $c_{ai}$ are \textit{n-ary} constraints,
\ie $|S_{ai}| \geq 2$. This means that preferences are specified for
each individual analysis decision, while consistencies only make sense
when considered between the analysis decision of two or more
coordinating \glspl{sas}. Then also note that dividing
$\mu_{A}(\cdot)$ into two sub-objectives, with two associated sets of
constraints, has two advantages: firstly, it ensures the separation of
concerns between consistency and preferences, and, secondly, it
guarantees increased privacy with respect to preferences, because the
$c_{pi}$ must not be shared with other \gls{sas}
\cite{Greenstadt_2007}.

\begin{figure}[t]
  \centering
  % \includegraphics[draft, width=\linewidth, height=6cm]{Figure.pdf}
  \input{figures/analysiscoord_v2.tex}
  \caption{Example of \ACDCOP involving two
    \glspl{sas}. \textbf{Legend:} $x_1$ and $x_2$ are variables,
    $c_1$, $c_2$, $c_3$ are constraints, $a_1$ and $a_2$ are agents,
    $\mathit{cadapt}$ means \textit{coordinated adaptation},
    $\mathit{ladapt}$ is \textit{local adaptation}, and
    $\mathit{nadapt}$ is \textit{no adaptation}.}
  \label{fig:Analysis_DCOP}
\end{figure}

\textbf{Example.} \reffig{fig:Analysis_DCOP} depicts the \dcop
formalization of an example \ACDCOP involving two coordinating
\gls{sas}. In this example, \textbf{SAS 1} strongly prefers
adaptation; this is specified by the $c_{p1}$ constraint, which
assigns a cost of $\infty$ to the \textit{no adaptation}
decision. $c_{p1}$ also specifies that \textbf{SAS 1} slightly prefers
\textit{coordinated adaptation} over \textit{local adaptation} by
assigning a lower cost to the former. In the case of \textbf{SAS 2},
$c_{p2}$ expresses a strong preference for \textit{no adaptation}.
Finally, the consistency constraint $c_{a1}$ specifies that it is not
valid for only one of the \gls{sas} to decide on \textit{coordinated
  adaptation}. In this example, the resulting optimal assignments, \ie
that minimizes $\mu_A(\cdot)$, would be $\sigma^* = \{\mathit{ladapt},
\mathit{nadapt}\}$, where the first value corresponds to $x_{a1}$ and
the second to $x_{a2}$.

%% \textbf{\Glspl{coordpointA}} map to the set $X_a =
%% \{x_{a1},\dots,x_{an}\} \subseteq \mathbf{X}$; the domain of each
%% $x_{ai}$ is $D_{ai} = \{\mathit{ldev}, \mathit{gdev},
%% \mathit{ndev}\}$, where $\mathit{ldev}$ corresponds to \textit{local
%%   deviation}, $\mathit{gdev}$ to \textit{global deviation}, and
%% $\mathit{ndev}$ to \textit{no deviation}.

%% \textbf{\Glspl{coordpointAPC}} map to the set $X_t =
%% \{x_{t1},\dots,x_{tn}\} \subseteq \mathbf{X}$; for each $x_{ti}$ we
%% have the domain $D_{ti}=\{\mathit{cadapt, ladapt, nadapt}\}$, where
%% $\mathit{cadapt}$ corresponds to \textit{coordinated adaptation},
%% $\mathit{ladapt}$ to \textit{local adaptation}, and $\mathit{nadapt}$
%% to \textit{no adaptation}.

%% Next, we specify the \textbf{\gls{coordobjective}} of \ACDCOP using
%% a \dcop objective function $\mu_{A}$ defined as follows:

%% \begin{equation}
%%   \mu_{A}(\sigma) = \sum_{c_{ai} \in F_a} c_{ai} (\sigma_{S_{ai}}) + \sum_{c_{ti} \in F_t} c_{ti} (\sigma_{S_{ti}}) + \sum_{c_{pi} \in F_p} c_{pi} (\sigma_{S_{pi}}) \,,
%% \end{equation}

%% where $F_a,F_t,F_p \subseteq \mathbf{F}$ are the sets of constraints,
%% with $c_{ai} \in F_a$ ensuring the consistency between multiple
%% \glspl{coordpointA}, $c_{ti} \in F_t$ ensuring the consistency between
%% \glspl{coordpointA} and \glspl{coordpointAPC},

\iffalse

Next, we formally specify analysis coordination \mapef{AC} as a
\dcop. We call the resulting specification \ACDCOP. To aid system
designers in constructing an \ACDCOP, we provide in this section a set
of application-independent specification primitives, \ie patterns. The
\ACDCOP specification primitives are summarized in Table ... and
explained in more details below.


\textit{Adaptation decision variables} express the need for an adaptation.
More concretely, they express the triggering the planning activity. 
The domain of adaptation decision variables can be
as simple as $\{adapt, \neg adapt\}$.
Yet, more nuanced decision are also supported, \eg trigger a special kind of 
planning activity. 
Each \gls{sas} owns \am{owns?} at least one adaptation decision
variable.
\am{what would be a situation for more than 1 variable? example?}

\textit{Adaptation decision constraints} represent the consistency
constraints between adaptation decision variables. 
\am{unclear whether this is only locally or also already relevant for coordination}
The adaptation
decision constraints guard against conflicts, \eg
only one \gls{sas} is allowed to carry out adaptations due to
environmental coupling, but also to promote synergies, \eg it is
sufficient if adaptation is carried out by a single
\gls{sas}. 
\am{a little too shallow; can you elaborate what env coupling is etc}
Adaptation decision constraints will output a high cost,
\eg $\infty$, if some assignments of the adaptation decision variables
involved in the constraint are incompatible, and a low cost,
otherwise.
\am{you have not introduced the notion of cost before; IMHO you should do when introducing DCOP above; also, it may be very misleading as we used cost also in our running example}

\textit{Adaptation decision preferences} are unary constraints
representing the preference of a \gls{sas} for the different possible
assignments of owned adaptation decision variables.  \gls{sas} employ
adaptation decision preference constraints to specify the perceived
trade-off between the expected utility of carrying adaptations and its
expected cost.
\am{sorry, really did not get it :-(}
\am{also, concerning the association: you introduce 1:1, but actually the classes would inherit an *-* constraint association from the DCOP superclasses, or? Is this feasible to model it in such a way? Maybe it becomes clearer when using association names/labels}

\textit{Planning coordination triggers} are variables representing the
decisions of \glspl{sas} to proceed with planning coordination or to
restrict themselves to local planning only. The domain of such
variables is the set $\{trigger, \neg trigger\}$. Each \gls{sas}
owns at least one planning coordination trigger.

\textit{Planning coordination preferences} are unary constraints
representing the preference of a \gls{sas} for participating
in planning coordination.

\textit{Planning coordination consistency constraints} are constraints
between multiple planning coordination triggering variables or between
planning coordination triggering variables and adaptation decision
variables. Such constraints ensure decision consistency between
multiple \gls{sas}. Note that both the variables and the constraints
mentioned above are conditioned on the states of either the managed
system itself or of its environment and are updated at \runtime based
on the available monitoring information.

\am{not shown in figure, explain} The \textit{objective function} is the \textit{sum} of constraints and
the \dcop is a minimization problem.
\am{does each agent have its own objective fct?}

Following the standard definition of a \dcop (Section
\ref{sec:Back_DCOP}), variables are each owned by a single
\textit{agent} and each \textit{agent} owns a single variable. 
\am{really? i.e., a 1:1 mapping from agent to variable?}
Agents
belong logically to their corresponding \gls{sas}, with the
\glspl{sas} being responsible for assigning the computation
carried out by agents to concrete software and hardware
resources\am{now all of a sudded you mention something concrete like sw, hw; how does it related to the running example?}\footnotemark{}.

\footnotetext{We note that, in practice, agents are simply computer
  programs implementing a certain \dcop algorithm and they jointly
  solve \dcops by exchanging messages.}

To illustrate the definitions and concepts enumerated above, we apply
them in specifying the analysis coordination \mapef{AC} in the \cloud
computing scenario discussed in \refsec{sec:Running_Example}.


% We start by
% specifying the analysis coordination \mapef{AC} problem
% (\reffig{fig:Analysis_DCOP}):

Our specification considers two \textit{adaptation decision
  variables}, $a_1$, associated to the infrastructure \gls{sas}, and
$a_2$ owned by the application \gls{sas}. The two variables share the
same domain, \ie $D_{a_1} = D_{a_2} = \{adapt,\neg adapt\}$. Note
that, in \reffig{fig:Analysis_DCOP}, $a^1_1 = a^1_2 = adapt$ and
$a^2_1 = a^2_2 = \neg adapt$.  
\am{suggest simplifying / making it more readable as follows:}
Note
that, in \reffig{fig:Analysis_DCOP}, $a_\textrm{inf} = a_\textrm{app} = adapt$ and
$\xbar{a}_\textrm{inf} = \xbar{a}_\textrm{app} = \neg adapt$.  
Similarly, we specify the
\textit{planning coordination triggers} with two variables, $T_1$ and
$T_2$, having the same domain
$D_{T_1} = D_{T_2} = \{trigger, \xbar{trigger}\}$.

\am{this sounds strange; you model the situation to respond to the concrete scenario; but you would need to model preference in general, independent of the concrete scenario; maybe changing the order helps: (1) explain preference in principle; (2) show that it addresses the scenario}
Next we specify the \textit{adaptation decision preferences}. As
introduced in \refsec{sec:Running_Example}, the application \gls{sas}
is experiencing a decrease in user satisfaction, while
the infrastructure \gls{sas} experiences an increase in operational
costs. We assume that this situation translates to higher preference
for adaptation, which, in turn, means assigning, in the corresponding
constraints, lower costs to the $adapt$ variable assignment than to
the $\xbar{adapt}$ one. The concrete costs are depicted in
\reffig{fig:Analysis_DCOP}, in constraints $c_5$ and $c_7$.

In the case of \textit{planning coordination preferences}, we assume
that the current states of the managed system and of its environment
do not affect the preference for planning coordination. However, we
assume that there is a slight adversity towards coordinating planning,
\eg due to the communication overhead. The concrete constraints,
$c_6$ and $c_8$ are depicted in \reffig{fig:Analysis_DCOP}.\am{sorry, but nothing concrete in Fig 4; still just the variables c ;-)}
\am{I think this figures needs much more explanation; what do the matrices mean? How is what is shown here mapped to the formalization from above? Who (owner of app vs infra) is expressing which part of the DCOP? The part that is within the grey boxes is clear, but what about the boundary ones and the ones outside the grey boxes?}

Further, we specify the \textit{adaptation decision constraint},
denoted by $c_1$ in \reffig{fig:Analysis_DCOP}. The constraint $c_1$
represents in this case expected benefit of adapting both managed
systems. As mentioned in \refsec{sec:Running_Example}, we consider
that the current situation requires exploiting the synergies between
the application \gls{sas} and the infrastructure \gls{sas}, therefore
we assign the lowest cost to the assignment
$\{a_1 = adapt, a_2 = adapt \}$.

For \textit{planning coordination consistency constraints}, we first
assume that, if one \gls{sas} requires planning coordination,
the other must participate as well. To specify this requirement, we
introduce constraint $c_4$, which assigns a cost of $0$, \ie
\textit{consistent}, to $\{T_1 = trigger, T_2 = trigger\}$ and
$\{T_1 = \xbar{trigger}, T_2 = \xbar{trigger}\}$, and $\infty$,
otherwise (\reffig{fig:Analysis_DCOP}). Next, based on the situation
described in \refsec{sec:Running_Example}, we consider that the
application \gls{sas} wishes to engage in planning coordination if the
managed system requires adaptation, therefore we construct the costs
in $c_3$ accordingly. Contrary, the infrastructure \gls{sas} does not
have strong consistency requirements, therefore $c_2$ will output the
cost of $0$ for any joint assignment of $a_1$ and $T_1$.

As explained above, each variable is assigned to an agent. In
our example system, the infrastructure \gls{sas} owns an agent for
$a_1$ and one managing $T_1$, \ie $A_{a_1}$ and $A_{T_1}$. Similarly,
the application \gls{sas} owns agents $A_{a_2}$ and $A_{T_2}$.
\am{hmmm.... I think this I did not get above; so you have more than one agent per SAS? why?}

As the objective function for the DCOP \am{is there a single one, or one per SAS?}, we choose the sum of constraints. \am{why?}
With
this, the analysis coordination \mapef{AC} problem is fully specified
as a \dcop. The two \gls{sas} can now solve the \dcop by
calling a \dcop solver. 
\am{each one solver of their own? maybe this part should be explained in the POC section}
The selection of \dcop solver can be done
based on the criteria briefly mentioned in \refsec{sec:Back_DCOP} and
discussed in detail in \cite{Fioretto_2018}. For example, by applying
the DPOP solver [cite], we obtain the following optimal assignment of
variables:

\todo Show DPOP variable assignment results for the example.

\am{this addresses somewhat my above comment; (a) I would not put as final rmark, but move upfront to say that we assume this for the running example, (b) you should address this again in the discussion when you discuss the applicability of the technique in practice!} As a final remark, it is important to note that, while we specified
above analysis coordination \mapef{AC} from a centralized perspective,
in practice, specifying coordination as \dcop is done collaboratively
by the system designers or administrators of the two
\gls{sas}. Specifically, the system designers or administrators must
agree on the following points:
\begin{enumerate*}
\item the general problem structure, \ie number of variables and
  constraints,
\item the \dcop objective function,
\item the weight of constraints in the \dcop objective for ensuring
  fairness, and
\item the \dcop solver.
\end{enumerate*}
We leave the protocols through which system designers or
administrators agree on these points to future work.

\begin{figure}[t]
  \centering
  % \includegraphics[draft, width=\linewidth, height=6cm]{Figure.pdf}
  \input{figures/analysiscoord.tex}
  \caption{\gls{dcop}-based analysis coordination \mapef{AC} applied to the running example from \refsec{sec:Running_Example}. \todo Update constraint values.}
  \label{fig:Analysis_DCOP}
\end{figure}

\fi

\subsection{Realizing \PCDCOP with \dcop} \label{sec:Coord_P}

\iffalse
\begin{figure}[t]
  \centering
  % \includegraphics[draft, width=\linewidth, height=6cm]{Figure.pdf}
  \input{figures/planningtypes.tex}
  \caption{Planning coordination metamodel. \todo Add a box for ``Agent''.}
  \label{fig:PlanningTypes}
\end{figure}


\begin{figure}[t]
  \centering
  % \includegraphics[draft, width=\linewidth, height=6cm]{Figure.pdf}
  \input{figures/planningcoord.tex}
  \caption{\gls{dcop}-based planning coordination \mapef{PC} applied to
    the running example from \refsec{sec:Running_Example}. \todo Update constraint values.}
  \label{fig:Planning_DCOP}
\end{figure}

\fi

Here we specify \PCDCOP with \dcop, following the conceptual elements
described in \refsec{sec:ConceptualArch}. We begin with the
\glspl{coordpoint}. We specify \textbf{\glspl{coordpointPstate}} as
\dcop variables from the set $X_{ps} =\{x_{ps1},\dots,x_{psn}\}
\subseteq \mathbf{X}$. The domain of each $x_{psi}$ is
$D_{psi}=\{\mathit{state}_{i1},\dots,\mathit{state}_{in}\} \subseteq
\mathbf{D}$, where $\mathit{state}_{ij}$ describes a particular state
$j$ of the \gls{sas}
$\mathtt{S_i}$. Similarly, we specify the
\textbf{\glspl{coordpointPaction}} as variables from $X_{pc}
=\{x_{pc1},\dots,x_{pcm}\} \subseteq \mathbf{X}$, with domains
$D_{pai}=\{\mathit{aspace}_{i1},\dots,\mathit{aspace}_{I'm}\}
\subseteq \mathbf{D}$. Here, $\mathit{aspace}_{ij}$ denotes a possible
action space $j$ of a \gls{sas} $\mathtt{S_i}$. Note that we do not
make any implicit assumption regarding the correspondence between
states and action spaces, \eg it can be that multiple action spaces
are allowed in a particular state (this is achieved with the
\gls{coordconstPPA}).

We can now specify the \textbf{\gls{coordobjective}} of \PCDCOP using
a \dcop objective function $\mu_{P}$ given by:

\begin{equation}
  \begin{alignedat}{2}
  \mu_{P}(\sigma) =& \quad\mu_{s}(\sigma) + \mu_{c}(\sigma) + \mu_{sc}(\sigma) &+& \mu_{sp}(\sigma) + \mu_{cp}(\sigma)  \\
  =& \sum_{\substack{c_{si} \in F_s \\ i=1..|F_s|}} c_{si} (\sigma_{S_{si}})
  &+& \sum_{\substack{c_{ci} \in F_c \\ i=1..|F_c|}} c_{ci} (\sigma_{S_{ci}}) \\
  +& \sum_{\substack{c_{sci} \in F_{sc} \\ i=1..|F_{sc}|}} c_{sci} (\sigma_{S_{sci}})
  &+& \sum_{\substack{c_{spi} \in F_{sp} \\ i=1..|F_{sp}|}} c_{spi} (\sigma_{S_{spi}}) \\
  +& \sum_{\substack{c_{cpi} \in F_{cp} \\ i=1..|F_{cp}|}} c_{cpi} (\sigma_{S_{cpi}})
  \end{alignedat}
\end{equation}

where $\mu_{s}(\cdot)$ is the \gls{coordconstP}, $\mu_{c}(\cdot)$ is
the \gls{coordconstPA}, $\mu_{sc}(\cdot)$ is the \gls{coordconstPPA},
$\mu_{sp}(\cdot)$ is the \gls{coordconstPpref}, and $\mu_{cp}(\cdot)$
is the \gls{coordconstPApref}. $F_s, F_c, F_{sc}, F_{sp}, F_{cp}
\subseteq \mathbf{F}$ are sets of constraints. Consistencies are
specified with the constraints $c_{si} \in F_s$ between two or more
\gls{coordpointPstate}, $c_{ci} \in F_c$ between two or more
\gls{coordpointPaction}, and $c_{sci} \in F_{sc}$ each between one
\gls{coordpointPstate} and one \gls{coordpointPaction}. State
preferences are specified with the constraints $c_{spi} \in F_{sp}$,
while action preferences are specified with $c_{cpi} \in F_{cp}$.  The
assignments $\sigma_{S_{si}}$ and $\sigma_{S_{sp}}$ correspond to
variables from $X_{ps}$, $\sigma_{S_{ci}}$ and $\sigma_{S_{cp}}$
correspond to variables from $X_{pc}$, and $\sigma_{S_{sci}}$
correspond to variables from both $X_{ps}$ and $X_{pc}$. As in
\ACDCOP, preference constraints are unary, while the consistency
constraints are n-ary.

Because in \PCDCOP we have two sets of variables, $X_{ps}$ and
$X_{pc}$, we define two corresponding sets of agents, namely $A_{ps}
\subseteq \mathbf{A}$ and $A_{pc} \subseteq \mathbf{A}$,
respectively. In line with the assumption introduced in
\refsec{sec:Back_DCOP}, each agent manages a single variable. It
follows that each \gls{sas} $\mathtt{S_i}$ owns two agents, $a_{psi}
\in A_{ps}$ and $a_{pci} \in A_{pc}$. While this might seem
conceptually bizarre, \ie why does one need two agents inside a
\gls{sas}, the constraints $c_{spi}$ guarantee, in fact, that the
decisions of one agent within a \gls{sas} are consistent with those of
the other agent. However, this might indeed introduce a performance
penalty as more messages must be exchanged within the \gls{sas}
\cite{yokoo2012distributed}. Regarding, the \textbf{peers} and
\textbf{algorithm} of \PCDCOP, the same considerations apply as in
\ACDCOP (\refsec{sec:Coord_A}).

\textbf{Example.} We apply \PCDCOP to a job dispatching system in
\refsec{sec:Experimental}.

\iffalse

\textit{Coordination points} are variables representing preconditions,
postconditions, allowed set of actions, future system state, or
planning goals, with the concrete meaning being specific to a system's
design. If the system requires planning over \textit{time horizons},
the coordination points will consist of sequences of preconditions,
postconditions, etc. Each \gls{sas} participating in \mapef{P}
coordination defines and manages its own set of coordination points.

\textit{Coordination constraints} represent consistency requirements
between coordination points and between coordination points and input
variables. Assuming a minimization problem, the coordination
constraints will assign $\infty$ to inconsistent coordination point
settings and $0$ to consistent coordination point settings. Note that
coordination constraints assign positive real values different
from $0$ to specify a preference ordering over a joint assignment of
compatible coordination points.

\textit{Coordination preference constraints} are unary constraints
specifying the preference ordering of a \gls{sas} over settings
of its own coordination points.

\textit{Agents} managing input variables handle the communication and
protocol implementation for the \mapef{A} and \mapef{M} components,
while coordination points are managed by \textit{agents} of the
\mapef{P} components participating in the \plancoord
activity.

The \textit{objective function} is the \textit{sum} of constraints and
the \dcop is a minimization problem.

We illustrate the concepts and definitions introduced in this section
by applying them to the example scenario described in
\refsec{sec:Running_Example}.

We start with specifying the coordination points. We define two
coordination point variables, one for the infrastructure \gls{sas},
\ie $p_1$, and one for the application \gls{sas}, \ie $p_2$.  The
domain of the infrastructure \gls{sas} coordination point variable
represents the two possible provisioning strategies, that is
$D_{p_1} = \{p^1_1, p^2_1\} = \{performance, conservative\}$. The
coordination point of the application \gls{sas} has the domain
$D_{p_2} = \{p^1_2, p^2_2, p^3_2\} = \{low, medium, high\}$, the
values representing the possible \gls{qos} threshold settings of the
application managing subsystem. Each of the two variable is owned by a
different agent: the infrastructure \gls{sas} owns the agent managing
$p_1$ and the application \gls{sas} owns the agent managing $p_2$.

We specify the preferences of \gls{sas} towards the assignment of
planning coordination variables using coordination preference
constraints. Constraint $c_2$ describes the preference of the
infrastructure \gls{sas}; we assume that the infrastructure \gls{sas}
prefers the \textit{conservative} strategy because of its smaller
energy consumption, therefore $p^2_1$ has the lowest cost in the
$c_2$. The application \gls{sas} prefers to guarantee high levels of
\gls{qos}, \eg because it could result in higher profits, therefore
the $p^3_2$ assignment has the lowest cost in
$c_3$. \reffig{fig:Planning_DCOP} depicts the complete definition of
$c_2$ and $c_3$.

Lastly, we define the coordination constraint $c_1$ between $p_1$ and
$p_2$. We use $c_1$ to encapsulate the utility, with respect to
expected costs and user satisfaction, of the joint assignments of
$p_1$ and $p_2$. Here we assume that the
$\{p_1 = performance, p_2 = medium \}$ gives the best trade-off
between expected costs and user satisfaction to the two \gls{sas}.

As in the case of analysis coordination \mapef{AC}, the objective
function of the planning coordination \mapef{PC} \dcop is the sum of
constraints. The discussion on design-time agreements on problem
structure, objective function, and constraint fairness at the end of
the previous section also applies in the case of \mapef{P}
coordination.

\todo Show DPOP variable assignment results for the example.

In the next section, we experimentally validate our planning
coordination \mapef{PC} technique using a more complex application --
infrastructure coordination scenario.

\footnotetext{\textit{CSP+Planning} \cite{Nissim_2010} iteratively
  expands the number of available coordination points until agents can
  successfully produce local plans. In our work, we assume that there
  are enough coordination points available from the beginning.}

\fi

\subsection{Prototypical implementation} \label{sec:ProtoImpl}
\begin{figure*}[t]
  \input{figures/conceptualarch_class.tex}
  \caption{Simplified class diagram.}
  \label{fig:ClassDiagram}
\end{figure*}

We implement \CoordDCOP following the basic structure depicted in
\reffig{fig:ClassDiagram}. We define two classes, one for \ACDCOP and
one for \PCDCOP. The classes share a common interface, \ie
\texttt{\CoordDCOP{Activity}}, providing three methods:
\texttt{update()} for providing the \textit{input} to \CoordDCOP,
\texttt{trigger()} for triggering the actual coordination, and
\texttt{getSolution()} for extracting the coordination solution, \ie
values of \glspl{coordpoint}, after the coordination process has
finished. The classes \texttt{\ACDCOP} and \texttt{\PCDCOP} hold lists
of variables and constraints with the types described in
\refsec{sec:Coord_A} and \refsec{sec:Coord_P}, together with a list of
peers. Note that in \texttt{\PCDCOP} the variables and constraints
associated to \glspl{coordpointPaction} can be 0-or-more, instead
of 1-or-more; we consider that the \glspl{coordpointPaction} are
optional and not required in cases where coordinating on the allowed
action set is not important (see \refsec{sec:Experimental}).

The coordination algorithms of \ACDCOP and \PCDCOP are part of the
concrete \texttt{DCOPAgent} implementations. It is up to the users of
\CoordDCOP to select and implement the \dcop algorithms that best fit
their application-specific requirements. The selection of a \dcop
algorithm should be done following a trade-off analysis, \eg based on
the performance - solution quality described in
\cite{Fioretto_2018}. For the purposes of this paper, we chose DPOP
\cite{petcu2005dpop} as the underlying \dcop algorithm for the
\CoordDCOP agents. DPOP is an established \textit{complete} algorithm,
\ie it guarantees the participating agents always reaching a true
optimal solution, if such solution exists.

In our experiments (\refsec{sec:Experimental}), we use the DPOP
implementation from \pydcop \cite{rust2019pydcop}. \pydcop is a Python
library facilitating the easy and quick experimentation with \dcop: it
implements a number of established \dcop algorithms, \eg DPOP
\cite{petcu2005dpop}, Max-Sum \cite{Farinelli_2008}, or DSA
\cite{zhang2005distributed}, it handles the communication between
agents, and it provides useful performance metrics, \eg the number of
exchanged messages or the sizes of exchanged messages. Other \dcop
libraries exist, such as Frodo \cite{leaute2009frodo} or DisChoco
\cite{wahbi2011dischoco}, however, we chose \pydcop due to its modern
codebase\footnotemark{} and good integration within the larger Python ecosystem.

\footnotetext{https://github.com/Orange-OpenSource/pyDcop}


% We skip the monitoring and execution MAPE acitivities
\iffalse
\subsection{Coordinating the monitoring function}

\begin{figure}[t]
  \centering
  % \includegraphics[draft, width=\linewidth, height=6cm]{Figure.pdf}
  \input{figures/monitoringcoord.tex}
  \caption{\gls{dcop}-based analysis \mapef{M} decision coordination.}
  \label{fig:Monitoring_DCOP}
\end{figure}

As in the case of analysis coordination (\refsec{sec:Coord_A}), we
formulate \coordmon as two \dcops, an \forwardp, which addresses
\reqMone, as described in \refsec{sec:SOTA_M}, and a \backwardp
implementing \reqMtwo. The \forwardp takes as inputs raw monitoring
observations and models the cooperative reasoning of autonomic
managers over a notion of global system state. The \backwardp, on the
other hand, takes as inputs the out of the \forwardp and models
autonomic managers reasoning on the implications of a certain global
state on their local domains of responsibility.

Given the similarities to the analysis coordination, we briefly
present only the key differences between \coordmon \dcop primitives
and those introduced in \refsec{sec:Coord_A}. Thus, in the case of the
\forwardp:

\textit{Input variables} model raw monitoring observations and their
domain is constrained to a particular value by the \textit{input unary
  constraints}. \textit{Aggregation variables and constraints} model
distributed reasoning. \textit{Output variables and constraints} model
a notion of global system state. In the case of \coordmon,
\textit{agents} of all types of variables are assigned to \mapef{M}
components, with the distribution of agents to real sub-systems being
handled in the \coordman layer (\refsec{sec:Concept_Arch}). The same
logic applies to the \backwardp.

\subsection{Coordinating the execution function}

\begin{figure}[t]
  \centering
  % \includegraphics[draft, width=\linewidth, height=6cm]{Figure.pdf}
  \input{figures/executioncoord.tex}
  \caption{\gls{dcop}-based planning \mapef{E} coordination.}
  \label{fig:Exec_DCOP}
\end{figure}


% Case 2) is motivated by a natural question following the
% transaction-based adaptation execution protocol proposed in
% \cite{Weissbach_2017}: \textit{``what happens after execution fails
%   and the system is rolled-back to a safe state?''}.

% We model the \preexecp similarly to the planning coordination problem,
% that is, autonomic managers agree on the values of
% \textit{coordination points}. Coordination points represent both
% agreements on actuation actions, \ie what should be actuated and when,
% and also agreements on what would constitute a failure under the
% current adaptation plans. Coordinating on the meaning of failures can
% translate in practice to agreeing on parameters of failure handling
% methods, such as the one proposed in \cite{Weissbach_2017}. Next we
% detail the \dcop modeling primitives of the \preexp:

To address the coordination requirements defined in
\refsec{sec:SOTA_E}, we model execution \mapef{E} coordination as two
\dcops: a \preexecp, addressing \reqEone, and a \failurep, addressing
\reqEtwo.

We model the \preexecp similarly to the planning coordination problem,
that is, autonomic managers agree on the values of coordination
points, here called \textit{enactment coordination points}. Enactment
coordination points model agreement on actuation actions (what should
be actuated and when) and are constrained by means of preference and
consistency constraints. The input variables of the \preexecp are the
outputs of planning \mapef{P}, \ie local plans (\refsec{sec:Coord_P})

% The key difference is that we explicitly introduce two
% types of coordination points two support the two requirements
% described above:
% \begin{enumerate*}
% \item coordination points modeling agreement , and
% \item coordination points modeling agreement on what would constitute
%   a failure under the current adaptation plans and how such failures
%   should be handled.
% \end{enumerate*}
% Coordinating on the meaning of failures can translate in practice to
% agreeing on parameters of failure handling methods, such as the one
% proposed in \cite{Weissbach_2017}. Therefore, the \dcop modeling
% primitives of the \mapef{E} function are the following:

\iffalse

The primitives of the \preexecp are:

\textit{Input variables} are the outputs of planning \mapef{P}, \ie
local plans (\refsec{sec:Coord_P}). The domain of input variables
is given by the space of all possible plans.

\textit{Input unary constraints} restrict the value of input variables
to the actual local plan computed by \mapef{P}. The input unary
constraints assign $0$ to variable values representing the actual plan
and $\infty$ to all other values.

\textit{Enactment coordination points} represent, as introduced above,
agreements on actions. Such variables are required, for example, when
an adaptation can be enacted by multiple autonomic managers or when an
adaptation must be enacted by multiple autonomic managers and the
managers must coordinate on the correct sequence of actions.

\textit{Enactment constraints} model consistency constraints between
enactment coordination points and between enactment constraints and
input variables. Similarly to the planning coordination constraints
(\refsec{sec:Coord_P}), enactment constraints assign $\infty$ to
inconsistent joint enactment coordination point settings and $0$ to
consistent enactment coordination point settings. Note that
coordination constraints assign positive real values different than
$0$ to model a preference ordering over a joint assignment of
consistent enactment coordination points.

\textit{Enactment preference constraints} model the preferences of
individual autonomic managers over their own enactment actions, in
case a (local) adaptation can be fully realized by multiple actions
(or sequences of actions) of the same autonomic manager.

\fi

In the \failurep, autonomic managers agree on the values
of coordination points, which agreement coordination on what would
constitute a failure under the current enactment actions and how such
failures should be handled. Coordinating on failures can translate in
practice to agreeing on parameter settings of failure handling
methods, such as the one proposed in \cite{Weissbach_2017}. The \dcop
associated to the \failurep has the following primitives:

\textit{Input variables} represent both the enactment coordination
points mentioned above and system state information used to establish
context, \eg the outputs of \mapef{M} or \mapef{A} components.

\textit{Input unary constraints} restrict, as before, the input
variable domain to the actual, real values.

\textit{Failure definition coordination points} model, as introduced
above, agreements on what constitutes a failure. The domains of such
variables correspond to the possible parameter settings of failure
detection algorithms.

\textit{Failure definition constraints} have multiple roles:
\begin{enumerate*}
\item failure conditioning constraints between failure definition
  coordination points and input variables, defining which settings of
  input variables can lead to which failures,
\item failure consistency constraints between failure definition
  coordination points, determining which failures exclude other
  failures.
\end{enumerate*}
As before, $0$ assignments model consistency and $\infty$ assignments
model inconsistencies, assuming a minimization problem. Here, non-zero
or non-infinity assignments will not model preference, but the
likelihoods of certain failures occurring, given certain variable
settings (of inputs, enactment coordination points, failure
coordination points).

\textit{Failure handling coordination points} represent, as introduced
above, agreements on how a failure should be handled. The domains of
such variables correspond to the possible parameter settings of
failure handling algorithms, such as the one proposed in
\cite{Weissbach_2017}.

\textit{Failure handling constraints} model consistency checks
between failure handling coordination points, failure definitions,
input variables, and enactment coordination points, \ie they specify
that failure $F$ should be handled in this way given the current
context. The assignments of such constraints are similar to the ones
out the enactment constraints.

For both the \preexecp and the \failurep, the \textit{objective
  functions} are the sum of constraints, \ie they are minimization
\dcops, and \textit{agents} correspond to the involved \mape
components. While agents of enactment coordination points can be
easily assigned to the \mapef{E} components of individual \mape loops,
variables corresponding to failures are associated more to the state
of the whole system, therefore assigning their agents to sub-systems
is decided by the coordination management layer (Section
\refsec{sec:Coord_Man}).

Figure \ref{fig:Exec_DCOP} depicts an example \gls{dcop}-based
\mapef{P} coordination for the decentralization instance from Figure
\ref{fig:Coord_Control}. \todo Figures and maybe explanations.

Finally, we \textbf{summarize} the sequence of \gls{dcop}-based
coordination \mape loop activities in \reffig{fig:Planning_DCOP}. Note
that the figure also depicts activities that are not handled by our
method, namely reading or disseminating sensor readings, local
planning, and local actuation.

\begin{figure}[t]
  \centering
  % \includegraphics[draft, width=\linewidth, height=6cm]{Figure.pdf}
  \input{figures/activitycoord.tex}
  \caption{Overview of the coordination activities proposed in
    \refsec{sec:Decision_Coord.}.}
  \label{fig:Activity_DCOP}
\end{figure}

\fi


\iffalse

\section{Coordination management with DCOP} \label{sec:Coord_Man}

\todo Mention in \refsec{sec:Concept_Arch} that coordination
management is future work.

\fi

\clearpage



\newcommand*{\iprov}{A}
\newcommand*{\aprov}{B}

\section{Formalizing the coordination of multiple managing subsystems} \label{sec:CoordFormalization}

%% \begin{figure}
%%   \centering
%%   % \includegraphics[draft, width=\linewidth, height=6cm]{Figure.pdf}
%%   \input{figures/conceptualarch_v4.tex}
%%   \caption{My figure.}
%% %%   \label{fig:Conceptual}
%% \end{figure}

In this section we introduce a set-theoretic, domain-independent, and
solution-independent formalization of the coordination of multiple
managing subsystems in assemblies of \gls{sas}. Such a formalization
is important for reasoning about coordination in a
solution-independent way. Later in this work, we will show how to map
this coordination formalization to a \glsxtrfull{dcop}, with
coordination then becoming equivalent to solving the \gls{dcop}.

%in a decentralized way with an off-the-shelf algorithm.

The formalization we introduce next is similar to the ones proposed in
\cite{Glazier_2019,Glazier_2020,Abeywickrama_2020} and aims at
capturing the elements representing the state of the managed
subsystems, the configuration spaces of the managing subsystems, the
global and \gls{sas}-specific objectives of the assembly, together
with the knowledge and models relating configurations and states to
objective satisfaction.  Thus, given an assembly of $n$ \gls{sas},
where each \gls{sas} consists of a managed subsystem and managing
subsystem, we formalize the coordination of configurations between the
$n$ \glspl{sas} as the tuple $\langle S, C, O, K, \Sigma, \rho
\rangle$:

\begin{itemize}
\item $S = S_1 \times S_2 \times \cdots \times S_n$, where, given a
  \gls{sas} $i$, $S_i$ is the set of possible states of the managed
  subsystem $i$ and of its environment, as monitored by the managing
  subsystem $i$,
\item $C = C_1 \times C_2 \times \cdots \times C_n$, where $C_i$ is
  the set of possible configurations of the managing subsystem of
  \gls{sas} $i$,
\item $O = G \times O_1 \times O_2 \times \cdots \times O_n$, where
  $G$ is a set of possible global goals and $O_i$ are
  \gls{sas}-specific goals,
\item $K = K_1 \times K_2 \times \cdots \times K_n$, where $K_i$ is
  the \textit{knowledge} of SAS $i$, \ie the set of all possible
  models relating states from $S_i$ and configurations from $C_i$ to
  the satisfaction of goals from $O$,
\item $\Sigma = S \times C \times O \times K$ is the complete state of
  the system composed by the $n$ \glspl{sas},
\item $\rho: \Sigma \times C \to \mathbb{R^+}$, where $\rho(s, c')$
  gives the cost of the new configuration $c' = (c'_1, c'_2, \dots,
  c'_n) \in C$ of the $n$ \gls{sas}, given $s \in \Sigma$, the current
  state of the assembly.
\end{itemize}

The objective of coordination is then to find:

\begin{equation} \label{eq:CoordFormalObj}
c^\star = \argmin_{c' \in C} \rho(s, c').
\end{equation}

One can say that, essentially, the function $\rho(\cdot)$
\textit{predicts} the effect of switching the configurations of the
managing subsystems to $c'$ and associates to this effect a
cost. Employing the expectations surrounding the effect of change to
drive decision-making is a common practice in the self-adaptive
systems literature
\cite{Paucar_2016,Calinescu_2015,Anders_2015,Baresi_2019,Jahan_2020}.

Finally, We emphasize that $c^\star = (c^\star_1, c^\star_2, \dots,
c^\star_n) \in C$ is a globally-optimal solution and does not give
guarantees with respect to the optimal satisfaction of local,
\gls{sas}-specific goals. This means that one can encounter cases
where $c^\star_i$ does not optimally satisfy a local objective $O_i$.

%% We discuss how we can obtain $c^\star$ in a fully decentralized manner
%% using \dcop in the next sections.

\textit{Example.} We conceptually apply the formalization introduced
above to the \gls{cloud} exemplary scenario from
\refsec{sec:MotivationExmpl}. \reftab{tab:FormalizationExample}
depicts the mapping of informal adaptation concerns to formal sets.
$S_1$ formalizes the set of states that can be possibly monitored by
the managing subsystem of the application \gls{sas}, consisting of two
dimensions: the requests for static video assets, \ie Requests, and
the picture quality of served videos, \ie Quality. Similarly, $S_2$
formalizes the set of states that can be monitored by the
infrastructure \gls{sas}, consisting of a resource demand dimension,
\ie Demand, and of a provisioning dimension, \ie \glspl{vm}. We note
that the Users, Quality, Demand, and \glspl{vm} are subsets of
$\mathbb{N}$ or $\mathbb{R}$ and model quantities.

Further, $C_1$ is a set of possible configurations of the managing
subsystem of the application \gls{sas}: maximize-served-users, \ie
$C_U$, and satisfaction-maximization, \ie $C_S$. Similarly, $C_2$
formalizes the set configurations of the managing subsystem of the
infrastructure \gls{sas}: efficiency-oriented self-adaptation, \ie
$C_E$, and performance-oriented self-adaptation, \ie $C_P$.

The objectives of the two \gls{sas} are formalized as follows. The
application \gls{sas} objectives $O_1$ are given in two dimensions: a
demand dimension, \ie Users Target, and a user satisfaction dimension,
\ie Satisfaction Target. Similarly, the infrastructure \gls{sas}
objectives $O_2$ consider the demand on the infrastructure, \ie Demand
Target, and provisioning of resources, \glspl{vm} Target. In this
example, the sets constructing $O_1$ and $O_2$ can be numeric in
nature.

Finally, the knowledge set $K$ is given as follows. The knowledge set
$K_1$ of the application \gls{sas} is given in two dimensions: a
dimension of models relating the managing subsystem configurations to
the amount of users served and a dimension of models relating the
managing subsystem configurations to the satisfaction experienced by
the users served. Similarly, the knowledge set $K_2$ of the
infrastructure \gls{sas} is also given in two dimensions: one relating
the managing subsystem configurations to how well the application-level
demand is addressed and another dimension relating to

\begin{table}
  \caption{Coordination formalization with \CoordDCOP for the running
    example from \refsec{sec:MotivationExmpl}.}
  \label{tab:FormalizationExample}
  % BEGIN RECEIVE ORGTBL mapping
\begin{tabular}{lll}
\hline
Type & Application \gls{sas} & Infrastructure \gls{sas}\\
\hline
\(S = S_1 \times S_2\) & \(S_1 = \text{Users} \times \text{Quality}\) & \(S_2 = \text{Demand} \times \text{VMs}\)\\
\(C = C_1 \times C_2\) & \(C_1 = \{C_U, C_S\}\) & \(C_2 = \{C_E, C_P\}\)\\
\(O = O_1 \times O_2\) & \(O_1 = \text{Users Target}\, \times\) & \(O_2 = \text{Demand Target}\)\\
 & \(\qquad\quad \text{Satisfaction Target}\) & \(\qquad\quad \text{VMs Target}\)\\
\(K = K_1 \times K_2\) & \(K_1 = \text{Latency Models}\, \times\) & \(K_2 = \text{Energy Models}\)\\
 & \(\qquad\quad \text{Cost Models}\) & \\
\end{tabular}
% END RECEIVE ORGTBL mapping


%%   \begin{comment}
\iffalse
#+ORGTBL: SEND mapping orgtbl-to-latex
    |----------------------+--------------------------------------------+-----------------------------------------|
    | Type                 | Application \gls{sas}                      | Infrastructure \gls{sas}                |
    |----------------------+--------------------------------------------+-----------------------------------------|
    | $S = S_1 \times S_2$ | $S_1 = \text{Users} \times \text{Quality}$ | $S_2 = \text{Demand} \times \text{VMs}$ |
    | $C = C_1 \times C_2$ | $C_1 = \{C_U, C_S\}$                       | $C_2 = \{C_E, C_P\}$                    |
    | $O = O_1 \times O_2$ | $O_1 = \text{Users Target}\, \times$       | $O_2 = \text{Demand Target}$            |
    |                      | $\qquad\quad \text{Satisfaction Target}$   | $\qquad\quad \text{VMs Target}$         |
    | $K = K_1 \times K_2$ | $K_1 = \text{Latency Models}\, \times$     | $K_2 = \text{Energy Models}$            |
    |                      | $\qquad\quad \text{Cost Models}$           |                                         |

\fi
    %%   \end{comment}

\end{table}

\section{\Glsxtrlong{dcop}}

\Glsxtrfullpl{dcop} \cite{Modi_2005, Nguyen_Yeoh_2019,Fioretto_2018}
involve agents coordinating the value assignments of owned variables
in order to optimize a certain objective function. \dcops are related
to the \csp, a kind of formal specification often employed in the
self-adaptive literature, \eg in \cite{metzger2016coordinated, Paz_2016,
  Oliveira_2013, AlShara_2018, Bruneliere_2018, Song_2013,
  Anders_2015, Vansyckel_2013}. \dcops generalize \csps, \ie by
allowing constraints to take real values instead of, and also extend
them to the distributed or multi-agent setting.

%% The multi-agent system community has studied many applications of
%% \dcops to real-life problems, such as coordinating \glsxtrshort{iot}
%% devices to minimize energy consumption in smart grids
%% \cite{fioretto2017multiagent}, coordinating logistic operations using
%% privacy-sensitive means \cite{leaute2011coordinating}, minimizing
%% congestion in disaster evacuation scenarios
%% \cite{kinoshita2013effective}, composing web services in a
%% \gls{qos}-aware manner \cite{Temglit_2018}, placing application
%% components on \cloud resources \cite{Jin_2011}, or implementing the
%% self-repair function in networks of physical agents
%% \cite{rust2020resilient} (\todo maybe remove examples; they also
%% appear in the introduction).

In the multi-agent systems literature
\cite{Nguyen_Yeoh_2019,Fioretto_2018}, a \dcop is defined as a tuple
$\langle A, X, D, F, \pi, \mu \rangle$, where:

\begin{itemize}
  \item $A = \{a_1, \dots, a_n\}$ is the set of agents.
  \item $X = \{x_1, \dots, x_n\}$ is the set of variables.
  \item $D = \{D_1, \dots, D_n\}$ is a set of finite variable domains,
    with $D_i = \{d_{i1}, \dots, d_{ik}\}$ being the domain associated
    to variable $x_i$.
%%   \item the tuples $(x_i, d_i)$, where $d_i \in D_i$, are
%%     \textit{value assignments}; the set $\sigma = \{(x_i, d_i) |
%%     i=1..n\}$ is a \textit{complete assignment} of values to
%%     variables, while $\sigma_S \subseteq \sigma$ is called a
%%     \textit{partial assignment}.
  \item $F = \{f_1, \dots, f_m\}$ is a set of \textit{constraint
    functions}, also known as \textit{cost functions} or simply
    \textit{constraints}, where $f_i: D_{l} \times \cdots \times D_{k}
    \to \mathbb{R^+}$; it is said that each $f_i$ has a scope $S_i
    \subseteq X$; the role of a constraint is to map a partial
    assignment $\sigma_{S_i} \in D_{l} \times \cdots \times D_{k}$ of
    variables from its scope to a real-valued \textit{cost}. An
    important characteristic of a constraint function $f_i$ is its
    \textit{arity}\footnotemark{}, \ie how many variables are part of
    its scope $S_i$.

    \footnotetext{\dcop algorithms usually assume an arity of at most
      two, that is they only operate on \textit{unary} or
      \textit{binary} constraints. There have been extensions proposed
      to algorithms in order to handle n-ary constraints
      \cite{Pecora_2007}.}

      % Another common solution is to pre-process
      % the n-ary constraint into multiple binary or unary ones (cite).}
  \item $\pi : X \to A$ is a function mapping variables to agents. If
    $\pi(x_i) = a_i$, then it means that $a_i$ controls how the values
    from $D_i$ are assigned to $x_i$, \ie $a_i$ \textit{controls} or
    \textit{owns} $x_i$. Note that, for simplicity, \dcop algorithms
    usually assume that an agent controls a single variable and that a
    variable is controlled by a single agent\footnotemark{}. We follow
    the same assumption in this paper.

    \footnotetext{Techniques to work around this limitation are
      discussed in \cite{Modi_2005,yokoo2012distributed}.}

\item $\mu(\sigma)$ is the \textit{objective function}, where $\sigma
  \in D_1 \times \cdots \times D_n$ is a complete assignment. It is
  usually assumed that the objective function is just the sum of
  costs, \ie $\mu (\sigma) = \sum_{f_i \in F} f_i(\sigma_{S_i})$ -- a
  key assumption for many algorithms.
\end{itemize}

Solving the \dcop means finding a complete assignment $\sigma^{\star}$
such that:

\begin{equation} \label{eq:DCOPmuObjective}
  \sigma^{\star} = \argmin_{\sigma \in D_1 \times \cdots \times
    D_n} \sum_{f_i \in F} f_i(\sigma_{S_i})
\end{equation}

which minimizes\footnotemark{} the objective function
$\mu(\sigma)$. Solving a \dcop is known to be NP-hard
\cite{Fioretto_2018, Modi_2005}.

\footnotetext{Note that, for simplicity, all the \dcops discussed in
  this paper aim at minimizing an objective function. However, in
  general, \dcops can also be constructed as maximization problems. In
  maximization \dcops, constraint functions are known as
  \textit{reward functions} or \textit{utility functions}.}

Note that a \dcop is solved in a distributed way: agents exchange
messages with their neighbors\footnotemark{}, following certain rules
or \textit{algorithms} so as to discover the optimal assignment
$\sigma^{\star}$. Starting out as extensions of established discrete
optimization algorithms, \eg SyncBB \cite{hirayama1997distributed}
extending the branch-and-bound algorithm, many algorithms have
been proposed in the past two decades to solve \dcops, \eg
\cite{petcu2005dpop, Modi_2005, Farinelli_2008}. For a comprehensive
survey on \dcop algorithms, please see \cite{Fioretto_2018}.

\footnotetext{Two agents $a_1$ and $a_2$ controlling variables $x_1$
  and $x_2$ are \textit{neighbors} if $\exists c \in F$ with
  scope $S$ having the property that $x_1, x_2 \in S$.}

\section{Coordination as a \glsxtrlong{dcop}} \label{sec:MappingToDCOP}

Within assemblies of \glspl{sas}, \dcop can provide both the formal
language to describe complex coordination problems between multiple
\glspl{sas} and the necessary mechanisms to carry out the coordination
itself, via the \dcop algorithms. As explained earlier, in \CoordDCOP
we map the formal coordination specification introduced in
\refsec{sec:CoordFormalization} to a \dcop. Coordinating the managing
subsystems of the \glspl{sas} pertaining to the assembly becomes then
equivalent to solving the \dcop, \ie minimizing $\rho(\cdot)$ and
identifying the optimal configuration $c^\star$ from
\refeq{eq:CoordFormalObj} is equivalent to minimizing $\mu(\cdot)$
from \eqref{eq:DCOPmuObjective} and obtaining an optimal assignment to
the \dcop variables.


%% from \refeq{eq:CoordFormalObj}, \ie of minimizing $\rho(\cdot)$ and
%% identifying the optimal $c^\star$, to solving a \dcop, \ie minimizing
%% the $\mu(\cdot)$ objective.

To map the formal coordination specification from
\refsec{sec:CoordFormalization}, we propose a semi-manual, top-down
approach in which experts specify, starting from $\rho(\cdot)$, the
structure of a \dcop, including variables, agents, and constraints. At
\runtime, this \dcop will be updated dynamically, in an automated
fashion, to take into account the current complete state $s \in
\Sigma$ of the assembly of \glspl{sas} (see
\refsec{sec:CoordinationProcedure}). Solving the \dcop and obtaining
the optimal coordination solution $c^\star$ is carried out at \runtime
in a fully decentralized manner by employing a \dcop
algorithm. Mapping $\rho(\cdot)$ to a \dcop is detailed below.

\textit{Variables, domains, and agents.} Each $x_i \in X$ corresponds
to the configuration selection of the managing subsystem of \gls{sas}
$i$. The set of possible configurations $C_i$ is represented by the
domain $D_i$ of $x_i$. Agents $a_i$ controlling variables $x_i$ and
implementing \dcop algorithms are assumed to run in a trusted
execution environment pertaining to the administrative domain of each
\gls{sas} $i$.

\textit{Constraints.} The $\rho(\cdot)$ function is decomposed to
\dcop constraints, \ie to functions $f_i \in F$. In the decomposition,
we differentiate between unary constraints, \ie $f_i$ with scope
cardinality $|S_i| = 1$, and n-ary constraints, \ie $f_j$ with $|S_j|
> 1$. Considering a \gls{sas} $i$, we employ unary constraints, and
call them \textit{preference constraints}, to specify the negative
contribution\footnotemark{} of each configuration from $D_i$ to
$O$. Note that such negative contribution is calculated independently
of all the other variables of the \gls{dcop}, therefore preference
constraints, as their name implies, are suitable, for example, to
formally specify and quantify the preferences of stakeholders or
system designers for particular managing subsystem configurations. We
consider that each variable $x_i$ has at most one preference
constraint associated to it.

We employ n-ary constraints, and call them \textit{consistency
  constraints} to specify the joint negative contribution of
configurations pertaining to two or more \glspl{sas} to $O$. As their
name implies, consistency constraints are suitable to formally specify
and quantify how well two or more configurations work together. Thus,
consistency constraints can capture both conflicts and synergies
between the managing subsystem configurations of multiple \glspl{sas}.

\footnotetext{We use \textit{negative contribution} because we assume
  a minimization \gls{dcop}.}

Please note that, in theory, all preference constraints could be
merged into consistency constraints -- for a variable $x_i$, the
cost values given by its preference constraint could be simply summed
to those costs given by all consistency constraints $x_i$ is involved
in. However, the decomposition into two types of constraints achieves
better separation of concerns, potentially simplifying both the
design-time engineering process and the runtime update of the
\gls{dcop} given the evolving state of the assembly of
\gls{sas}. Moreover, extremely relevant for multi-stakeholder
scenarios, the decomposition into preference and consistency
constraints can have important privacy benefits: some of the
\gls{dcop} algorithms, \eg DPOP \cite{petcu2005dpop}, prescribe that
agents exchange information about constraint values only for n-nary
constraints and only with those other agents that are directly
involved in those constraints, while unary constraints stay private.

Finally, we note that system designers have a significant number of
options when deciding on a \dcop algorithm to realize coordination. In
their survey \cite{Fioretto_2018}, \citeauthor{Fioretto_2018} review
the theoretical properties of twelve \dcop algorithms and propose a
set of guidelines for the selection of \dcop algorithms. For example,
a system designer can take into account:

\begin{itemize}
\item the amount of available resources -- when memory is limited,
  but network communication is not constrained, then search-based
  algorithms, such as ADOPT \cite{Modi_2005}, are preferred over
  inference-based ones, such as DPOP \cite{petcu2005dpop},
\item the topology of the \dcop constraint graph -- if the number of
  cycles is low then DPOP can deliver optimal solutions efficiently or
  if the constraint graph is acyclic Max-Sum \cite{Farinelli_2008} can
  become an event better choice, or
\item the strictness of privacy considerations -- in some
  algorithms, such as DPOP, agents only communicate with direct
  neighbors, while in algorithms such as ConcFB \cite{Netzer_2012}
  agents might exchange messages with non-neighbors.
\end{itemize}

\begin{figure}[t]
  \centering
  % \includegraphics[draft, width=\linewidth, height=6cm]{Figure.pdf}
  \input{figures/coadapt_dcop_example.tex}
  \caption{A possible mapping of the coordination formalization from
    \refsec{sec:CoordFormalization} to a \gls{dcop} following the
    approach introduced in \refsec{sec:MappingToDCOP}.}.
  \label{fig:DCOPApplicationExample}
\end{figure}

\textit{Example.} We map the coordination formalization introduced in
\refsec{sec:CoordFormalization} for the running example from
\refsec{sec:MotivationExmpl} to a
\gls{dcop}. \reffig{fig:DCOPApplicationExample} depicts the resulting
\gls{dcop} in a graph-like representation; variables are depicted
using white rectangles, agents are depicted as gray rectangles, and
constraints are depicted as lines.

In mapping the coordination formalization to a \gls{dcop}, we define
first the \dcop variables and their domains as follows. There are two
variables, $x_1, x_2 \in X$. The variable $x_1$ corresponds to the
configuration selection of the application \gls{sas} and has the
domain given by the two possible configurations of the managing
subsystem, \ie $D_1 = C_1 = \{C_u, C_S\} \in D$. Variable $x_2$
corresponds to the configuration selection of the infrastructure
\gls{sas} and its domain is given by $D_2 = C_2 = \{C_E, C_P\} \in D$.


Next, we construct the constraints of the \gls{dcop}, with
\reffig{fig:DCOPApplicationExample} depicting a possible design of
preference and consistency constraints. For this, we define two
preference constraints, $f_1, f_2 \in F$. The preference constraint
$f_1$ assigns a real-valued cost to each element of $D_1$, while $f_2$
assigns a cost to each element of $D_2$. For the purposes of this
example, we assume that configurations with lower operational costs
are preferred over those offering better service or user
satisfaction. The consistency constraint $f_3$ assigns a high cost
when the managing subsystems of the two \glspl{sas} are both
efficiency-focused, reflecting the assumption that such situation
would lead to poor user satisfaction, as explained in
\refsec{sec:MotivationExmpl}. As a clarification, note that the
reasoning presented in this paragraph, as well as the concrete cost
values depicted in \reffig{fig:DCOPApplicationExample}, are
conditioned, in practice, on the current complete state of the
assembly of \glspl{sas} $s^i \in \Sigma$. If the system moves to
another state $s^j\,, i \neq j$, then the constraints $f_1,f_2,f_3 \in
F$ should be updated accordingly, \eg due to decreasing energy costs,
it has become preferable and possible to always serve high-quality
videos, thus increasing user satisfaction.

\section{Coordination procedure} \label{sec:CoordinationProcedure}

The coordination procedure with \CoordDCOP can be split into two main
phases: \designtime and \runtime. The following happens at
\designtime:

\begin{enumerate}
  \item The system designer formalizes coordination using the
    framework introduced in \refsec{sec:CoordFormalization}.
  \item The system designer maps the coordination formalization to a
    \dcop and decides on an appropriate \dcop algorithm by following
    the steps described in \refsec{sec:MappingToDCOP}.
  \item The system designer defines an \textit{update
    function}\footnotemark{} which map the \runtime states $s \in \Sigma$ of the
    system assembly to the \dcop in an automated fashion, \eg adds new
    variables or constraints upon \glspl{sas} entering or leaving the
    assembly, updates the domains of variables when more
    configurations become available, or updates the preference and
    consistency constraints based on new goals or knowledge about how
    different configurations interact with each other.
\end{enumerate}

\footnotetext{As the update functions depends strongly on the
  coordination problem at hand, we consider that it lies outside the
  scope of this paper.}

Then, at \runtime, periodically or event-triggered, \eg upon major
changes in the system:

\begin{enumerate}
\item The update function maps the current state $s \in \Sigma$ of the
  assembly to the coordination \dcop.
\item The managing subsystems follow the selected \dcop algorithm in
  order to solve the \dcop and obtain the new optimal configurations
  $c^* \in C$.
\item The managing subsystems enact the new configurations.
\end{enumerate}


==> sections/background.tex <==
% \section{Terminology and Problem Statement}
\section{Fundamentals} \label{sec:Background_Dec}

\todo Maybe say throughout the paper that \CoordDCOP addresses
distributed coordination for analysis and planning instead of
decentralized? This might the connection to \dcop more obvious.

This section explains relevant fundamentals of SAS and decentralization.
In particular, we provide a concise definition and differentiation between the concepts of \textit{communication}
and \textit{coordination}.
This helps us to clearly understand the roles of communication and coordination in the decentralization of each of the four MAPE activities.
\am{check:was MAPE already introduced}
Finally, we review two typical conceptual architectures of decentralized \gls{sas}, which we will augment with our solutions for coordination.

\subsection{Planning}

Planning is the synthesis of a sequence of actions, \ie a plan, to be
followed by a system in order to reach some desirable goal state,
starting from an initial state
\cite{lavalle2006planning,ghallab2004automated}. Plans can be
synthesized in an automated way using a planning algorithm, \ie a
planner, which takes as input a formal specification of a planning
problem \cite{ghallab2004automated}. In addition to simply producing a
feasible plan, \ie a plan that brings the system from an initial state
to its goal state, planners can also optimize plans for a secondary
criterion \cite{lavalle2006planning}, \eg use a minimal number of
actions in the plan or minimize the expected resource expenditure
associated to executing the plan.

\subsection{\Glsxtrfull{map}}

In some classes of systems, \eg large-scale \gls{p2p} systems
\cite{DAngelo_2020}, it is undesirable or impossible to carry out
planning within some centralized planning component. If this is the
case, system designers might opt for distributing planning over
multiple planning agents, \ie \glsxtrfull{map}. Distributing planning
to agents can be desirable, for example, when increased privacy or
autonomy are important, when no central planning authority can be
identified or agreed upon, when the planning problem can be decomposed
in smaller, loosely coupled sub-problems which be solved in parallel,
or when carrying out planning locally is important for quick reactions
during the operation of the system \cite{de2009introduction}. Such
benefits make \Gls{map} attractive for different application domains,
such as robotics \cite{rizk2019cooperative}, logistics
\cite{ye2020differentially}, or \gls{cloud} computing
\cite{premarathne2020trust}. However, such benefits come at the cost
of additional coordination and the possibly reduced quality of
resulting plans, \eg due to limited communication means
\cite{de2009introduction}.

\subsection {Cooperative \gls{map}}

A special case of \gls{map} is cooperative \gls{map} in which agents
collaborate in order to synthesize a joint plan that solves a common
goal \cite{Torreno_2017}. We note that, while agents have a common
goal, each agent can have different capabilities, \ie a different set
of actions at its disposal, or even different incomplete or local
views\footnotemark{} over the planning problem \cite{Torreno_2017}.

\footnotetext{Agents know the common goal of the planning problem,
  however they do not have access to the complete system state.}

To solve a cooperative \gls{map} problem, agents engage in coordinated
plan synthesis schemes or algorithms. Many such algorithms have been
proposed in recent years [cite]. In their survey \cite{Torreno_2017},
\citeauthor{Torreno_2017} classify cooperative \gls{map} algorithms
into two main categories:
\begin{enumerate*}
\item \gls{unthreaded}, and
\item \gls{interleaved}.
\end{enumerate*}

In the algorithms pertaining to 1), agents plan independently, but
they coordinate\footnotemark{} before or after planning. The purpose
of coordination can be to ensure that the resulting plans are
compatible and that they can be merged, \ie pre-planning coordination,
or to remove inconsistencies between existing plans before merging,
\ie post-planning coordination \cite{Torreno_2017}. An important
advantage of \gls{unthreaded} is that it has low communication
overhead. However, employing 1) is not always possible, because, in
practice, some planning problems cannot be split in
independently-solvable sub-problems \cite{Torreno_2017}.

On the other hand, algorithms employing \gls{interleaved} are
well-suited for solving complex planning problem, where there is
strong coupling between the planning sub-problems of individual
agents. Such algorithms involve continuous coordination between the
agents during the planning process and have the drawback of increased
communication overhead \cite{Torreno_2017}.

\footnotetext{Coordination is the exchange of information carried out
  by agents for ensuring compatibility between their activities
  \cite{Torreno_2017}.}

\subsection{Coordination as distributed constraint optimization}

\Gls{unthreaded} \gls{map} algorithms often employ distributed
constraint satisfaction or optimization techniques to guarantee the
compatibility and optimality of multi-agent plans
\cite{Fabre_2010,Nissim_2010,cox2009efficient}. To this end, these
algorithms translate the coordination problem to established formal
problem specifications, such as the \glsxtrfull{dcsp} [cite] or the
\glsxtrfull{dcop} [cite]. Coordination points, \ie time-ordered sets
of possible actions, together with their, preconditions and effects
(post-conditions), are translated into vectors of \gls{dcsp} or
\gls{dcop} variables; the causality relations between coordination
points, \ie the relations between the preconditions and effects of
different actions, are specified as \gls{dcsp} or \gls{dcop}
constraints\footnotemark{} \cite{Nissim_2010,cox2009efficient}. Once
the coordination has been formalized, the resulting \gls{dcsp} or
\gls{dcop} can be solved with an off-the-shelf solver, \eg [cite]. If
a solution is found, then we arrived to a set of compatible plans.

\footnotetext{Essentially, in this formulation, variables capture the
  variability in agent plans, while constraints ensure the
  compatibility between agent plans, constraining the variability.}
%% To check:
%% - Planning First,
%% - DPGM \cite{pellier:hal-00981656} - individual agents use CSP to check if constraints received from other agents are consistent with their plans,
%% - $\mu$-SATPLAN \cite{Dimopoulos_2012}, uses a SAT solver to check the consistency of plans, similar to DPGM,
%% - MAPR,
%% - PMR,
%% - CMAP,
%% - MAP-LAKT,
%% - MARC,
%% - ADP,
%% - DISTOPLAN \cite{Fabre_2010}, uses a distributed optimization algorithm Message Passing Algorithm (MPA) to ensure the compatibility and optimality of agent plans,
%% - A#,
%% - PSM,
%% - DPP,
%% - TFPOP

\subsection{Planning in \glsxtrlong{sas}}

In \glsxtrfull{sas}, planning is ...


\subsection{Self-Adaptive Systems}

\iffalse
\begin{figure}[t]
  \centering
  % \includegraphics[draft, width=\linewidth, height=6cm]{Figure.pdf}
  \input{figures/coordinatedcontrol.tex}
  \caption{The coordinated control pattern \cite{Weyns_2013,
      Quin_2021} (left) and an example instance of the pattern.}
  \label{fig:Coord_Control}
\end{figure}
\fi

% some text \message{The column width is: \the\columnwidth}
% The column width is: \the\columnwidth
% The column width is: \the\columnsep

A \gls{sas} can modify its own structure and behavior at runtime based
on its perception of the environment, of itself and of its
requirements.  Thereby, a \gls{sas} can automatically maintain its
quality requirements in the presence of dynamic environment
changes~\cite{Weyns_2020,MetzgerQMBP22}.

A \gls{sas} typically is structured into two main elements: the system
logic, a.k.a. the managed element, and the self-adaptation logic,
a.k.a. the autonomic manager\cite{Kephart_2003, Weyns_2013,
  Weyns_2020}. The well-established MAPE-K reference model for
\gls{sas} structures the self-adaptation logic into four main
conceptual activities that rely on a common knowledge base (K).  These
activities (M)onitor the system and its environment, (A)nalyze
monitored data to determine adaptation needs, (P)lan adaptation
actions, and (E)xecute these adaptation actions at
runtime~\cite{Weyns_2020}.  \am{I think it is important to include K
  and later also explain its role!, otherwise looks incomplete}

%% would refrain from stating this; a reviewer may read "assumption" and then ask what if the assumption is violated?
%Given the ubiquitousness of the \mape model, we
%assume in the rest of this paper that the managing subsystem is always
%realized by means of \mape loops.

\subsection{Decentralized Self-Adaptive Systems}

In a decentralized \gls{sas}, the conceptual activities of the MAPE-K
reference model are distributed across two or more self-adaptation
logics~\cite{deLemos_2013, Weyns_2013}. A decentralized \gls{sas} can
be constructed either from a previously centralized \gls{sas}, \eg to
improve some performance aspects of a large \gls{sas}, or by
coordinating multiple existing \gls{sas}, \eg to avoid conflicts
between adaptations. Note that, although \CoordDCOP supports both
types of decentralized \gls{sas}, for simplicity and clarity we will
discuss \CoordDCOP from the perspective of the latter.

\todo mention that a
decentralized \gls{sas} comes from a previously centralized \gls{sas}
that has been decentralized for performance reasons or that it
comprises multiple \gls{sas} that now wish to coordinate for different
reasons. \am{hmmm, here again I get the impression that you started
  from a centralized version and turned this into a decentralized
  version of MAPE; as I understood from our last call, I thought you
  were starting from different MAPEs for different systems -- needs
  clarification} \todo get rid of jointly; use the definition from
\cite{Quin_2021}. To jointly realize some or all of the
\glsxtrlong{mape} activities, \mape loops must \textit{interact}, \eg
exchange messages, do remote calls, or influence each other through
environmental coupling \cite{Quin_2021}.  \am{what does to jointly
  realize mean? why are they not realized independently? also, realize
  may be too low-level term at this stage; or phrased differently: I
  think interaction is needed at a much higher level, i.e., already
  when conceptualizing and designing}

\todo get rid of interactions. \citeauthor{Weyns_2013} conceptually
classify interactions based on the role they play in decentralized
\gls{sas}\cite{Weyns_2013}: \am{for me, this is not really helpful;
  some of them are not relevant (like the 1st - not relevant for
  decenatrliz.), and the 2nd and 3rd are super confusing, not clear
  how they differentiate}
\begin{enumerate}
\item interactions between the managing subsystem and the managed
  subsystem, so as to collect monitoring information and to enact
  adaptations,
\item interactions in pairs of \textit{different} \mape activities
  (\textit{inter-activity} interactions), pertaining to the same or
  multiple \mape loops, \eg \mapef{A} triggers adaptation planning
  \mapef{P} if adapting the managed system is required, and
\item interactions between multiple \mape loops, within a single \mape
  activity, with the purposes of communication and coordination
  (\textit{intra-activity} interactions).
\end{enumerate}

%% suggest leaving out; is obvious and not our scope, may rather confuse
%\footnotetext{Note that, independently of the adaptation logic, the
%  managed subsystem of a decentralized \gls{sas} can also consist of
%  multiple, possibly interacting, logical parts [cite], \eg the
%  constituent peers of a \gls{p2p} system [cite].}

As mentioned in \refsec{sec:Introduction}, two  kinds of interactions between self-adaptation logics can be differentiated:
\am{note: I think we should call the whole MAPE-K conglomerate \gls{sas} logic, while only calling out MAPE when we refer to the activties; this may make reading the paper easier).}

\textbf{Communication} refers to the interaction between \gls{sas} logics with the goal of sharing information.
%This shared information may be used by the involved \gls{sas} logics to establish a consistent view (e.g., of the managed subsystem or the environment).
%I may also be used or for propagating control flow\am{what does this mean?}.
Communication is the primary kind of interactions between decentralized monitoring and execution activities.\am{needs evidence}

For monitoring, communication helps establish a consistent view of the
managed subsystem.  This is used, for example, to disseminate
information on the experienced \gls{qos} in \gls{p2p} systems
\cite{Colombo_2022} and in systems of self-assembling web-services
\cite{Kumar_2018,DAngelo_2020}.  \am{a more natural example for me
  would have been something like establish a joint and consistent
  run-time model or "digital twin" (KNOWLEDGE)}

For execution, communication aids in the realization of transaction-based protocols, so as to ensure the atomic and consistent execution of adaptations \cite{Weissbach_2017}.
\am{and possible something like NNN}

\textbf{Coordination} refers to the interaction between \gls{sas} logics with the goal of joint decision-making.
%Such joint decision-making can help to avoid conflicts between adaptations of different \gls{sas} logics and it can help to exploit synergies among adaptations.
%% Leave out, not really needed
%\footnotetext{We note that \citeauthor{Weyns_2013} divide the
%  intra-activity interactions in \textit{delegation} and
%  \textit{coordination}. Under our terminology, delegation is a
%  special case of communication.}
Coordination is the primary kind of interactions between decentralized analysis and planning activities.\am{needs evidence}
Coordination helps reasoning about the state of the managed subsystem and
in jointly deciding if adapting the managed system is truly required,
\eg due to deviations from operating goals or
requirements. 

For analysis, coordination is useful, for instance, to trigger self-healing in (multi-agent) self-organizing systems \cite{Weyns_2008} or to discover state inconsistencies due to time-lag in client-server systems \cite{Yamagata_2019}.

For planning, coordination can come under the form of \textit{cooperative planning} or under that of \textit{\plancoord}.  
Works such as \cite{Mencagli_2014,
  Pilgerstorfer_2017} are examples of cooperative planning, where
interacting \mape loops plan for a common goal by jointly solving a
planning problem, \eg by means of multi-agent planning
\cite{Torreno_2017}. In contrast, \plancoord takes place before and /
or after \mape loops have produced their plans
\cite{Torreno_2017}. The purpose of \plancoord is for \mape
loops to agree on planning constraints, including preconditions,
postconditions, allowed set of actions, future system state, or
planning goals. Once the planning constraints have been defined,
individual \mape loops can produce plans locally using any available
planning algorithm, under the assumption that resulting local plans do
not require further coordination, \ie they are compatible
\cite{Nissim_2010,Torreno_2017}. An example of \plancoord applied in
decentralized \gls{sas} is the multi-level elasticity control strategy
for \gls{cloud} and \gls{fog} infrastructures and distributed data
stream processing applications proposed in \cite{Nardelli_2019}, where
an \textit{application manager} and an \textit{infrastructure manager}
coordinate on elasticity plans.

%In this paper, we provide a technique for coordination within the
%\mapef{A} activity (\refsec{sec:Coord_A}) and one for \plancoord,
%within the \mapef{P} activity (\refsec{sec:Coord_P}).

% In this paper, we focus on the latter type of interaction,
% specifically on coordination. As we mentioned in
% \refsec{sec:Introduction}, we differentiate between
% \textit{communication}, \ie the exchange of information between \mape
% loops to establish a consistent view of the managed subsystem, and
% \textit{coordination}, \ie joint decision-making as to avoid conflicts
% and exploit synergies between adaptations.

% \am{does decentrlization always imply
%   interaction?}  \am{Fundamental question: in principle there are two
%   settings: (1) We have ONE centralized adaptation logic that controls
%   multiple managed systems (and we want to split this logic for sake
%   of decentralization); (2) There are two adaptation logics, one for
%   each \gls{sas} (and they have been developed independently), and we want
%   to make sure they work together/coordinate -- IMHO we may want to
%   explain this, especially whether we call it ONE \gls{sas} or multiple
%   \gls{sas}?}

% \am{do we need this here: if at all, move to intro}A
% decentralized management logic is often required in the case of large
% and dynamic system in order to implement hierarchies of control
% \cite{Baresi_2019} or manage interactions between peers
% \cite{DAngelo_2020, Colombo_2022}.

\iffalse
\subsection{Architectural patterns for decentralized \gls{sas}}
\todo get rid of this section.

\am{I guess this will be moved to a later part of the paper?}
Designers of decentralized \gls{sas} have many architectural options
when designing \mape-based managing subsystems, including: how many
\mape loops form the managing subsystem, what kind of interactions
take place between the \mape loops or between the \mape loops and the
managed subsystem(s), is there any control hierarchy between the \mape
loops, which of the decentralized \mape activities require active
coordination etc. Any such design decisions must be taken based on an
understanding of engineering trade-offs, including those affecting
scalability, robustness, responsiveness, or the inherent division of
administrative domains, among others \cite{Weyns_2013}.

With respect to design decisions for decentralized \gls{sas}, prior
works have observed that certain recurring \textit{architectural
  patterns} emerge in practice \cite{Weyns_2013, Quin_2021}. Out of
the five patterns identified in \cite{Weyns_2013}, two are strongly
coordination-intensive and addressed by our paper: the
\textit{regional planner} pattern and the \textit{coordinated control}
pattern.

The regional planner pattern characterizes decentralized \gls{sas}
requiring the strong separation of administrative domains or regions,
\ie parts of the \gls{sas} are managed by different
\textit{owners}. Regions are managed by their own \mape loops, however
cross-region coordination in the \mapef{P} activity is also carried
out to ensure the consistency of adaptation plans. The regional
planner can be encountered in federated \gls{cloud} computing where
\gls{cloud} providers coordinate the provisioning of computational
resources for improving costs or \gls{qos} \cite{Carlini_2016, Nallur_2013}.

The coordinated control pattern is typical to highly-distributed
systems where no controlling authority can be identified or agreed
upon \cite{Weyns_2013}, \eg in \gls{p2p} systems. The coordinated
pattern involves intra-activity interactions in the case of all four
\mape activity and thus is both communication- and
coordination-intensive. In practice, the coordinated control pattern
appears in fully-decentralized applications, such as autonomic service
assembly \cite{grassi2013qos}.

\todo Move to approach. To conceptually represent the patterns of
decentralized control and to promote systematic study of decentralized
\gls{sas}, a special graphical notation has been introduced in
\cite{Weyns_2013, Quin_2021}. Using this notation, one can specify

The notation is similar to a UML class diagram

\iffalse
\citeauthor{Weyns_2013} define three types of
interactions between \mape loops \cite{Weyns_2013}:

\begin{description}
\item [Managed-managing subsystem interactions] occur when a
  higher-level \mape loop acts as the management subsystem of a
  lower-level \mape loop, \ie the first \mape loop implement the
  adaptation logic, while the second loop is subjected to adaptation.
\item [Inter-component interactions] occur between \mape
  components (or functions) of different types, \eg between \mapef{M}
  and \mapef{A} or \mapef{P} and \mapef{E}, belonging to different
  \mape loops.
\item [Intra-component interactions] occur between \mape
  components (or functions) of the same type, \eg between \mapef{A}
  and \mapef{A} or \mapef{P} and \mapef{P}, belonging to
  different \mape loops.
\end{description}


\am{unclear why you introduce what follows; is it needed to elaborate the problem? is it needed later on in the paper, then consider moving to the place where you need it}

In their work, \citeauthor{Weyns_2013} observe that, with respect to
the interactions between \mape loops, certain structures of
 self-adaptive systems recur in the literature
\cite{Weyns_2013}. \citeauthor{Weyns_2013} derived a set of
\textit{decentralization patterns} to characterize such recurring
structures, namely the coordinated control, information sharing,
regional planning, hierarchical control, and \masterslave patterns.

While coordination patterns abstract away details regarding the actual
communication and coordination mechanisms, in their recent work
\cite{Quin_2021}, \citeauthor{Quin_2021} observe that, in practice,
certain interactions between \mape loops tend to be realized in
recurring ways. With this in mind, \citeauthor{Quin_2021} augment the
decentralization patterns introduced in \cite{Weyns_2013} with a
\textit{decentralization protocol}, \eg client-server,
publish-subscribe, market mechanisms, or gossiping, and a
\textit{decentralization channel}, \eg intermediary, remote call, or
direct messaging. For instance, \citeauthor{Quin_2021} note that
regional planning is most often implemented as a market mechanism
supported by direct messaging.

\fi

\todo Delete the rest of the section \refsec{sec:Background_Dec}.

\fi

\subsection{Communication vs coordination of \gls{sas}}
As a decentralized \gls{sas} consist of two or more interacting adaptation logics, here we more precisely define what interacting means.
The interaction between the adaptation logics consist of two dimensions:

First, \textit{communication}, which involves
the exchange of knowledge among decentralized \gls{sas}.
The main purpose of communication is to establish a consistent view of the managed subsystem\am{see above: do we have one system or many?} and thus can form the basis of adaptation decision-making
\cite{Weyns_2013}. \am{maybe link to KNOWLEDGE of Mape?}
Communication in \gls{sas} can be realized via mechanisms such as publish-subscribe, gossiping, and client-server architectures. \cite{Weyns_2013,Quin_2021} \todo give examples.

Second, \emph{coordination }, which is about joint
decision-making and joint problem-solving. 
\am{elaborate}
Coordination helps avoid conflicting decisions
and exploiting potential synergies. \todo give examples
Coordination in \gls{sas} can be realized by mechanisms such as market mechanisms \am{auctions?}, negotiation protocols, and distributed constraint satisfaction and optimization\cite{Weyns_2013,Quin_2021,MORE} .

\subsection{Coordination in decentralized \mape
  loops} \label{sec:Back_Coord_MAPE} Designers of \gls{sas} employ
coordination techniques in decentralizing the analysis \mapef{A} and
the planning \mapef{P} activities of the \mape loop.\am{why only AP and not ME? Needs explanation or references; or: do we need to make this claim at all?}

\am{IMHO should go to related work} Within the \mape loop, the role of the analysis \mapef{A} activity is
to decide, based on state information, both on whether the managed
subsystem has deviated from operating goals and requirements, and on
whether correcting the deviation mandates an adaptation
\cite{Kephart_2003}. Therefore, in actual \gls{sas}, the
implementation of the \mapef{A} activity can take various forms of
complexity, ranging from simple comparators [cite], to complex \csp
solvers \cite{AlShara_2018}. In the \gls{sas} literature, the
\mapef{A} activity has been decentralized over multiple \mape loops
for applications such as triggering self-healing in self-organizing
multi-agent systems \cite{Weyns_2008} or predicting state
inconsistencies due to time-lag in client-server systems
\cite{Yamagata_2019}.

\todo When discussion \mapef{P}, use the same examples in both
paragraphs.

\am{IMHO should go to related work} The planning function \mapef{P} is responsible for deciding how and
when an adaptation should be performed to correct deviations of the
managed system from operating goals or requirements
\cite{Weyns_2013}. In their mapping study \cite{Quin_2021},
\citeauthor{Quin_2021} have observed that planning is one of the most
often decentralized components of the \mape loop. For example, in the
context of \cloud computing, \citeauthor{Carlini_2016}
\cite{Carlini_2016} propose a technique for coordinating the
distribution of services between federated \cloud infrastructures,
while \cite{Nallur_2013} proposes an auction-based mechanisms for
application managers to coordinate on service composition.

\am{better in related work?; if you leave here, you should say which of the two is the focus of the paper ;-)}For the purposes of this work, we distinguish between
\textit{cooperative planning} and \textit{\plancoord}.  Works such as
\cite{Mencagli_2014, Pilgerstorfer_2017} are examples of cooperative
planning, where agents or autonomic managers plan for a common goal by
jointly and iteratively solving a planning or optimization problem. In
contrast, \plancoord is an activity taking place before and / or after
agents have produced their plans \cite{Torreno_2017}. Planning
coordination can be a standalone activity or integrated in a
cooperative planning process. An example of \plancoord applied in
decentralized self-adaptive systems is the multi-level elasticity
control strategy from \cite{Nardelli_2019}. Here,
\citeauthor{Nardelli_2019} propose a technique where an autonomic
manager of a data stream processing application coordinates on
elasticity plans with the autonomic manger of a computing
infrastructure.
% In
% the coordinated control pattern, for example, intra-component
% interactions occur between all components of coordinating \mape
% loops. \reffig{fig:Coord_Control} depicts the coordinated control
% pattern.

% \begin{itemize}
%   \item Coordinated control - requires intra-component interactions
%     between all components of coordinating \mape loops and are
%     typically encountered in systems such as...
%   \item Information sharing - involves coordination between the
%     \mapef{m} components of interaction \mape loops and characterize
%     systems such as ...
%   \item \masterslave - typical to systems such as ..p., where the
%     \mapef{A} and \mapef{P} functions centralized while the \mapef{M}
%     and \mapef{E} components are implemented by decentralized
%     workers. \pd{Pattern originally called Master/Slave, however the
%       trend nowadays is to ``soften'' such terminology. Not sure if we
%       should do it as well, given that we are not the authors of these
%       patterns}.
%   \item Regional planning - requires that monitoring, analysis, and
%     execution are carried out locally, while planning is delegated to
%     a centralized \mapef{P} component, with such a pattern being
%     typical to ...
%   \item Hierarchical control - typical to complex systems such as ...,
%     the pattern depicts the managing subsystem as a layered hierarchy
%     of \mape loops connected by managing-managed subsystems
%     interactions.
%   \end{itemize}





==> sections/discussion.tex <==
%% \section{Discussion} \label{sec:Discussion}

\section{Limitations}

We consider that the limitations of our approach mostly stem from the
choice of \dcop as a coordination model. Classical \dcop does not
explicitly handle or model concerns such as uncertainty in agent
action outcomes or knowledge, asymmetry and fairness in constraint
values, or uncooperative behavior of some agents. However, many of
these limitations have been addressed by the multi-agent community by
extending the \dcop formalization and devising specialized algorithms.
We did not consider the existing \dcop extensions in this paper, but
we leave them to future work.

Another limitation of our work is that we did not provide details on
the function of the \layerCoordMan. The \layerCoordMan plays an
important role in monitoring the effectiveness of coordination and
adjusting the coordination mechanism in order to meet some performance
targets. With respect to \dcop, adjustments of the coordination
mechanisms could mean: changes in constraints or variables, changes in
the objective function, or switching to a different \dcop algorithm
exhibiting different solution quality - performance trade-off. How to
carry out all these operations in an automated and effective manner is
an interesting research question and the subject of future work.

\TODO{Citations for importance and challenges in defining
  multi-stakeholder utility functions: \cite{Wohlrab_2022}}

\TODO{Mention that in practice the interaction process between
  \glspl{sas} must be formalized and verified, \eg by means of
  choreographies \cite{Guedemann_2016,Calinescu_Autili_2017}}

\TODO{Cite when talking about fairness of coordination
  \cite{Farahani_2021}}

\am{important that stakeholders still need to agree on some minimal information to model the DCOP!}


==> sections/introduction.tex <==
\newcommand{\gap}[1]{(\textbf{GAP#1})}
\newcommand{\gapone}{\gap{1}\xspace}
\newcommand{\gaptwo}{\gap{2}\xspace}
\newcommand{\gapthree}{\gap{3}\xspace}

\section{Introduction} \label{sec:Introduction}

There is a vast amount of work on how to engineer the adaptation logic
of \gls{sas}, such as rule-based adaptation
\cite{Ghahreman_2018,Mann_2021}, learning-based adaptation
\cite{Russo_2018,DAngelo_2020,MetzgerQMBP22,Feit_2022},
optimization-driven
\cite{Calinescu_2015,AlShara_2018,Chen_Bahsoon2_2017}, or
control-theoretic approaches
\cite{Baresi_2019,Filieri_2017,Camara_2020}, among others. The
majority of existing work focuses on realizing the adaptation logic in
a \textit{centralized} way, \ie as a single logical unit or controller
which oversees the adaptation of relevant system
components. Increasingly common is to organize the adaptation logic as
a single feedback loop with differentiated activities, \ie the \mape
loop reference model \cite{Kephart_2003}. However, such centralized
adaptation logic has a number of clear shortcomings: it exhibits a
single point of failure, has performance issues in the case of large
scale systems, and assumes total control over system components
\cite{Yang_Yi_2019} [more citations]. These limitations can prohibit
the adoption of centralized adaptation logic in some classes of
system, such as in the large-scale and highly-heterogeneous
Cloud-to-Edge systems [cite].

In contrast to the centralized case, in \textit{decentralized}
\gls{sas} responsibilities pertaining to the adaptation logic are
shared between two or more components \cite{deLemos_2013, Weyns_2013}.
Such decentralized adaptation logic is necessary for large-scale,
distributed, and multi-stakeholder \gls{sas}, where no
suitable centralized controller can be identified or agreed upon
[citations]. The adaptation logic of decentralized \gls{sas} is
commonly engineered as multiple interacting \mape loops
\cite{Weyns_2013}. Each \mape loop is either responsible for a
different adaptation concern, \eg \gls{qos} [cite], self-healing
[cite], or responsible for a different part of the \gls{sas}, \eg for
a different peer in a peer-to-peer system [cite].

In a decentralized \gls{sas}, \mape loops interact by
\textit{communicating}, \ie exchanging information, and by
\textit{coordinating}, \ie taking joint decisions. (\todo Revise what
follows to match Background.) While in centralized \gls{sas}, the
adaptation logic assumes a global view over the system, in
decentralized \gls{sas}, \mape loops communicate in order to establish
a common, consistent view of the system or its environment, on which
to base adaptation decisions. In the context of the \mape loop, the
monitoring \mapef{M} and execution \mapef{E} activities are
communication-driven. For example, communication during the \mapef{M}
activity most often entails exchanging state information [cite], while
in the \mapef{E} activity \mape loops can communicate failures in
adaptation enactment [cite]. (\todo Maybe say why we don't focus on
communication, \ie ``There are many communication techniques, \eg A,
B, C. We invite the reader to check \cite{Quin_2021} for a survey on
recent approaches.'')

In contrast to centralized \gls{sas}, which can directly take global
adaptation decisions, decentralized \gls{sas} employ coordination in
order to avoid conflicts, \eg [...], or to exploit synergies in
adaptation decisions, \eg [...]. In the \mape loop, the analysis
\mapef{A} and planning \mapef{P} activities are coordination-driven.
By coordinating in the \mapef{A} activity, interacting \mape loops
decide if the \gls{sas} requires adaptation and which parts of the
\gls{sas} should be adapted [cite]. On the other hand, \mapef{P}
coordination helps \mape loops to agree on planning constraints, such
as the allowed set of adaptations, post-conditions, or pre-conditions
[cite].

Initial prior works have shown how to realize coordination in some
concrete classes of decentralized \gls{sas} and for concrete
applications, \eg using market mechanisms to adapt resource
provisioning in federated \gls{cloud} infrastructures
\cite{Nallur_2013, Eisele_2022}, using multi-agent \gls{rl} to adapt
dependency realization in service-oriented computing
\cite{DAngelo_2020}, or constraint optimization for ...  However,
because existing work is closely tied to concrete applications, it is
not straightforward how to transfer the previously proposed
coordination techniques to new classes of decentralized
\gls{sas}. This limitation of existing work has been previously noted
in the self-adaptive systems literature and numerous calls have been
made for principled and systematic approaches to realizing
coordination in \gls{sas} [cite]. In practice, the lack of systematic
and application-independent design approaches can prohibit the
adoption of state-of-the-art techniques or lead to ad-hoc and
under-performing solutions.

\TODO{Also for MARL \cite{Galkin_2022}}

In this paper, we propose an application-independent,
formally-grounded coordination technique for decentralized \gls{sas}
based on \textit{distributed constraint optimization} \cite{Modi_2005,
  Nguyen_Yeoh_2019,Fioretto_2018}. A \gls{dcop} is an established and
well-studied problem setting from the field of multi-agent systems in
which agents coordinate to optimally assign values to the variables
they own. \Glspl{dcop} have shown great potential in solving a number
of real-world problems, including minimizing energy consumption in
smart grids \cite{fioretto2017multiagent}, coordinating logistic
operations \cite{leaute2011coordinating}, minimizing congestion in
disaster evacuation scenarios \cite{kinoshita2013effective}, or
placing application components on cloud resources \cite{Jin_2011}.

For decentralized \gls{sas}, \dcop enables system designers to specify
coordination problems between interacting \mape loops using a concise
formal language. The \dcop formalization is similar to other
constraint programming languages, often employed in the \gls{sas}
literature [cite examples]. A coordination problem, once specified as
a \dcop, can be efficiently solved using a variety of off-the-shelf
solvers \cite{fioretto2017multiagent}. \dcops enable fully
decentralized coordination, thus addressing many of the limitations of
centralized control, \eg having single point of failure, high
communication and computational requirements, and limited flexibility
and scalability \cite{Yang_Yi_2019}. In contrast to other coordination
techniques, such as multi-agent \gls{rl} and game-theoretic
approaches, \dcop solvers can exploit the problem structure, \eg peers
coordinate only with immediate ``neighbors'', to reach good solutions
in less time \cite{fioretto2017multiagent}.

Our contribution in this paper is twofold. Firstly, we propose an
application-independent reference architecture extending the \mape
feedback loop with two new activities: a \textit{planning
  coordination} \mapef{PC} activity and an \textit{analysis
  coordination} \mapef{AC} activity. In the \mapef{PC} activity,
\gls{sas} jointly decide on optimal planning constraints with the goal
of avoiding conflicts and exploiting synergies. The \mapef{AC}
activity enables \gls{sas} in jointly deciding if adaptations should
be carried out and if adaptation planning requires coordination, thus
avoiding the communication-intensive \mapef{PC} when not required. Our
second major contribution is that we provide a set of
application-independent specification constructs and primitives which
aid system designers in specifying \mapef{PC} and \mapef{AC} as
\dcops.

Below, \refsec{sec:Background} reviews the relevant \sota in
decentralized self-adaptive systems and the introduces the fundamental
theoretical concepts of \dcop. \refsec{sec:Decision_Coord} presents
our \gls{dcop}-based coordination technique. \refsec{sec:Experimental}
describes our experimental evaluation in the Simdex exemplar
\cite{Krulis_2022} and the obtained experimental
results. \refsec{sec:Discussion} presents a critical discussion of our
technique. \refsec{sec:Related_Work} describes how our technique
relates to existing approaches.


==> sections/stateoftheart.tex <==
\newcommand{\req}[2]{(\textbf{R#1#2})}
\newcommand{\reqMone}{\req{M}{1}\xspace}
\newcommand{\reqMtwo}{\req{M}{2}\xspace}
\newcommand{\reqAone}{\req{A}{1}\xspace}
\newcommand{\reqAtwo}{\req{A}{2}\xspace}
\newcommand{\reqAthree}{\req{A}{3}\xspace}
\newcommand{\reqPone}{\req{P}{1}\xspace}
\newcommand{\reqEone}{\req{E}{1}\xspace}
\newcommand{\reqEtwo}{\req{E}{2}\xspace}



\section{State-of-the-art analysis} \label{sec:SOTA}

In this section, we analyze the decentralized self-adaptive systems
literature and derive a set of coordination requirements for all four
functions of the \mape loop.

\iffalse
\subsection{Monitoring} \label{sec:SOTA_M}

Monitoring \mapef{M} is the part of the managing system responsible for
collecting information about the managed system itself and its
operating environment \cite{Weyns_2013}. In the context of
decentralized self-adaptive systems, monitoring is the most commonly
decentralized component of the \mape loop, as part of the information
sharing, \masterslave, and coordinated control decentralization
patterns \cite{Quin_2021}. For example, in \cite{DAngelo_2020}, the
authors propose a solution to the self-adaptive service assembly
problem in which autonomic managers exchange information about the
\textit{quality} of managed services in order to guide local assembly
planning. In \cite{Colombo_2022}, \citeauthor{Colombo_2022} propose a
\gls{p2p} and adaptive monitoring scheme aimed at fog computing
\cite{Yousefpour_2019}, in which fog nodes with \textit{follower}
roles collect local information on hardware and network utilization
and share it with their \textit{leaders}.

For the purposes of this work it is important to distinguish between
monitoring decentralization as \textit{information sharing} and as
\textit{\coordmon}. In contrast to information sharing
\cite{DAngelo_2020, Colombo_2022}, \coordmon refers to
decentralization schemes in which autonomic managers must
cooperatively reason about raw monitored values in order to resolve
uncertainty in monitoring information or to deduce higher-level
concepts. For example, in the context of assisted living, the authors
of \cite{Pecora_2007} demonstrate how \dcop-based solutions can infer
high-level human activities, \eg eating or taking medication, by
fusing information from location and posture detection sensors. In
their recent work \cite{Petrovska_2021}, \citeauthor{Petrovska_2021}
argue that aggregating monitoring observations is essential to
resolving uncertainty and conflicts for decentralized adaptive
\gls{cps} and propose an aggregation method based on subjective
logic\footnotemark{}.

\footnotetext{We note that \citeauthor{Petrovska_2021}
  \cite{Petrovska_2021} place the aggregation and reasoning over
  monitoring observations in the \mapef{A} component. However, we
  consider that, in general, tasks such as resolving uncertainty and
  reasoning about a global state should belong to the \mapef{M}
  function, while \mapef{A} is strictly responsible for deciding upon
  the need of adaptation. Regardless, we agree that it is not always
  straightforward to clearly separate the \mapef{M} and \mapef{A}
  components.}

In this work we choose to present a \gls{dcop}-based solution only to
\coordmon, as \dcop is an approach to modeling decentralized reasoning
and not a solution to information sharing. In alignment with works
such as \cite{Pecora_2007} and \citeauthor{Petrovska_2021}, we
consider that \coordmon requires both reasoning about the
\textit{aggregation} of locally-available information in order to
determine a higher-level system state \reqMone and
\textit{distributing} globally-available information in order to
derive local state \reqMtwo.

\fi

\subsection{Analysis} \label{sec:SOTA_A}

Within the \mape loop, the role of the analysis function \mapef{A} is
to decide, based on the managed subsystem state and its environment,
whether the managed system has deviated from operating goals and
requirements, and whether correcting the deviation mandates an
adaptation \cite{Kephart_2003}. In the self-adaptive systems
literature, the analysis component has been decentralized over
multiple \mape loops for applications such as triggering self-healing
in self-organizing multi-agent systems \cite{Weyns_2008} or predicting
state inconsistencies due to time-lag in client-server systems
\cite{Yamagata_2019}.

In this work, we decentralize the analysis function following a
\gls{dcop}-based approach, aiming to cover three potential analysis
requirements: \reqAone analysis decisions (local or global) can depend
solely on monitoring information, \reqAtwo analysis decisions (local
or global) can depend on both monitoring information and the analysis
decisions of other \mapef{A} components, and \reqAthree local analysis
decisions, \eg trigger local adaptations or raising alarms, depend on
some global analysis decision, \eg a global alarm state computed as
part of \reqAtwo.


\subsection{Planning} \label{sec:SOTA_P}

The planning function \mapef{P} is responsible for deciding how and
when an adaptation should be performed to correct deviations of the
managed system from operating goals or requirements
\cite{Weyns_2013}. In their mapping study \cite{Quin_2021},
\citeauthor{Quin_2021} have observed that planning one of the most
often decentralized components of the \mape loop. For example, in the
context of cloud computing, \citeauthor{Carlini_2016}
\cite{Carlini_2016} propose a method to coordinate the distribution of
services between federated cloud infrastructures, while
\cite{Nallur_2013} proposes an auction-based mechanisms for
application managers to coordinate on service composition.

For the purposes of this work, we must distinguish between
\textit{cooperative planning} and \textit{\plancoord}.  Works such as
\cite{Mencagli_2014, Pilgerstorfer_2017} are examples of cooperative
planning, where agents or autonomic managers plan for a common goal by
jointly and iteratively solving a planning or optimization problem. In
contrast, \plancoord is a information sharing or optimization activity
that takes place before and / or after agents have produced their
plans \cite{Torreno_2017}. \plancoord can be a standalone activity or
integrated in a cooperative planning process. An example of \plancoord
applied in decentralized self-adaptive systems is the multi-level
elasticity control strategy for \gls{cloud} and \gls{fog}
infrastructures and distributed data stream processing applications
proposed in \cite{Nardelli_2019}, where an \textit{application
  manager} and an \textit{infrastructure manager} coordinate on
elasticity plans.

% In this work we strictly focus on \plancoord and do not
% discuss its implications on cooperative planning, leaving this subject
% to future work.

In this work we strictly focus on \plancoord \reqPone and do not
discuss its implications on cooperative planning. Although distributed
constraint reasoning is sometimes used as a solution concept
\cite{Nissim_2010}, cooperative planning is a complex topic and
entails different types of modeling constructs and algorithms
\cite{Torreno_2017}, therefore we leave its study to future
work. However, we do consider that \gls{dcop}-based \plancoord is
sufficient to tackle a significant number of real problems, such as
those mentioned in \refsec{sec:Back_DCOP}.

% energy consumption minimization in smart grids
% \cite{fioretto2017multiagent}, web-service composition
% \cite{Temglit_2018}, application component placement \cite{Jin_2011},
% or implementing self-healing functionality \cite{rust2020resilient}.

\iffalse

\subsection{Execution} \label{sec:SOTA_E}

Within the \mape loop, the execution \mapef{E} function implements the
role of enacting adaptation plans on the managed system
\cite{Weyns_2013}. In \cite{Quin_2021}, the authors have observed that
\mapef{E} is most often decentralized as part of \masterslave pattern
instances. For example, in their approach to resource allocation and
placement of application containers on \gls{mec} infrastructures,
\citeauthor{Baresi_2019} \cite{Baresi_2019} propose, as part of their
solution, the partitioning of edge topologies into
\textit{communities}, each community having a \textit{leader}. A
global \textit{supervisor} manages and possibly adapts the structure
of communities in reaction to system or environmental changes, \eg
edge nodes are enabled or disabled. Re-structuring plans are forwarded
to community leaders who are responsible for executing them.

We note that, in general, the complexity of the execution function
\mapef{E} is given by the interaction possibilities with the managed
system, \ie available actuators. It can be that, in certain systems,
the role of \mapef{E} is to trigger certain actions according to a
given plan, \eg triggering user alerts \cite{Calinescu_2021}, while in
other systems execution is a very complex activity, \eg re-configuring
computing infrastructures \cite{Baresi_2019}. Moreover, in some
classes of decentralized self-adaptive systems, carrying out the
\mapef{E} activity entails further coordination among autonomic
managers. In \cite{Weissbach_2017}, the authors discuss in detail the
challenges associated to the coordinated execution of adaptations and
proposed a transaction-based protocol to ensure consistent adaptation
execution under message loss and failures in carrying out local
adaptations.

In this work we aim at supporting reasoning in the execution \mapef{E}
function of the \mape loop by covering two requirements: \reqEone
coordination required in order to implement complex adaptations or
actuations of the managed system, and \reqEtwo coordination in order
to define both what constitutes an execution failure and how failures
should be handled.

\fi
